Observations of the Naked-Eye GRB 080319B: Implications of Nature's Brightest Explosion

The first gamma-ray burst (GRB) confirmed to be bright enough to be seen with the naked eye, GRB 080319B at redshift z = 0.937, allowed for exquisite follow-up observations across the electromagnetic spectrum. We present our detailed optical and infrared observations of the afterglow, consisting of over 5000 images starting 51 s after the GRB trigger, in concert with our own analysis of the Swift data. The event is extreme not only in observed properties but intrinsically: it was the most luminous event ever recorded at optical and infrared wavelengths and had an exceedingly high isotropic-equivalent energy release in gamma-rays. At early times, the afterglow evolution is broadly consistent with being reverse-shock dominated, but then is subsumed by a forward shock at around 1000 s. The overall spectral energy distribution, spanning from ultraviolet through near-infrared wavelengths, shows no evidence for a significant amount of dust extinction in the host frame. The afterglow evolution, however, is highly chromatic: starting at about 1000 s the index shifts blueward before shifting back to the red at late times. In our deepest late-time observations, we find tentative evidence for an optical jet break and a luminous supernova. Finally, we examine the detectability of such events with current and future facilities and find that such an event could be detected in gamma-rays by BAT out to z = 10.7 (8 sigma), while the nominal EXIST sensitivity would allow detection to z ~ 32. At K band, this source would have been easily detected with meter-class telescopes to z ~ 17.

==> phot_all.tex <==

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Observations of GRB\,080319B\label{tab:photlogptel}}
\tablecolumns{5}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
  307.8 & {\rm J}     &    7.8 & $10.071 \pm 0.048$\tablenotemark{x} & $149073.3\pm  6451.0$\tablenotemark{x} \\
  316.0 & {\rm J}     &    7.8 & $10.100 \pm 0.048$\tablenotemark{x} & $145237.8\pm  6285.0$\tablenotemark{x} \\
  324.0 & {\rm J}     &    7.8 & $10.166 \pm 0.048$\tablenotemark{x} & $136684.7\pm  5914.8$\tablenotemark{x} \\
  344.0 & {\rm J}     &    7.8 & $10.389 \pm 0.048$ & $111255.0\pm  4815.5$ \\
  352.3 & {\rm J}     &    7.8 & $10.483 \pm 0.048$ & $102084.5\pm  4419.0$ \\
  360.2 & {\rm J}     &    7.8 & $10.563 \pm 0.048$ & $ 94763.2\pm  4102.4$ \\
  380.1 & {\rm J}     &    7.8 & $10.652 \pm 0.048$ & $ 87313.1\pm  3779.8$ \\
  388.4 & {\rm J}     &    7.8 & $10.722 \pm 0.048$ & $ 81846.4\pm  3544.3$ \\
  396.3 & {\rm J}     &    7.8 & $10.781 \pm 0.048$ & $ 77538.9\pm  3357.8$ \\
  416.3 & {\rm J}     &    7.8 & $10.877 \pm 0.048$ & $ 70983.9\pm  3074.6$ \\
  424.5 & {\rm J}     &    7.8 & $10.896 \pm 0.048$ & $ 69752.5\pm  3021.6$ \\
  432.4 & {\rm J}     &    7.8 & $10.952 \pm 0.048$ & $ 66227.7\pm  2868.9$ \\
  452.4 & {\rm J}     &    7.8 & $11.000 \pm 0.048$ & $ 63381.1\pm  2745.9$ \\
  460.7 & {\rm J}     &    7.8 & $11.082 \pm 0.048$ & $ 58776.0\pm  2546.7$ \\
  468.6 & {\rm J}     &    7.8 & $11.137 \pm 0.048$ & $ 55862.4\pm  2420.8$ \\
  488.6 & {\rm J}     &    7.8 & $11.266 \pm 0.048$ & $ 49636.3\pm  2151.9$ \\
  496.9 & {\rm J}     &    7.8 & $11.244 \pm 0.048$ & $ 50633.7\pm  2195.1$ \\
  504.8 & {\rm J}     &    7.8 & $11.314 \pm 0.048$ & $ 47485.4\pm  2059.2$ \\
  525.8 & {\rm J}     &    7.8 & $11.432 \pm 0.048$ & $ 42575.5\pm  1846.9$ \\
  534.1 & {\rm J}     &    7.8 & $11.447 \pm 0.048$ & $ 41991.4\pm  1821.5$ \\
  542.0 & {\rm J}     &    7.8 & $11.471 \pm 0.048$ & $ 41073.3\pm  1781.4$ \\
  561.9 & {\rm J}     &    7.8 & $11.589 \pm 0.048$ & $ 36863.8\pm  1599.6$ \\
  570.2 & {\rm J}     &    7.8 & $11.598 \pm 0.048$ & $ 36535.9\pm  1585.4$ \\
  578.2 & {\rm J}     &    7.8 & $11.602 \pm 0.048$ & $ 36391.5\pm  1579.1$ \\
  598.2 & {\rm J}     &    7.8 & $11.671 \pm 0.048$ & $ 34160.1\pm  1483.1$ \\
  606.4 & {\rm J}     &    7.8 & $11.694 \pm 0.048$ & $ 33441.0\pm  1452.1$ \\
  614.4 & {\rm J}     &    7.8 & $11.714 \pm 0.048$ & $ 32827.6\pm  1425.8$ \\
  634.4 & {\rm J}     &    7.8 & $11.675 \pm 0.048$ & $ 34053.3\pm  1478.4$ \\
  650.6 & {\rm J}     &    7.8 & $11.749 \pm 0.048$ & $ 31786.3\pm  1380.5$ \\
  670.6 & {\rm J}     &    7.8 & $11.950 \pm 0.048$ & $ 26424.1\pm  1148.8$ \\
  678.9 & {\rm J}     &    7.8 & $11.931 \pm 0.048$ & $ 26902.9\pm  1170.4$ \\
  686.8 & {\rm J}     &    7.8 & $11.978 \pm 0.048$ & $ 25749.0\pm  1119.9$ \\
  706.8 & {\rm J}     &    7.8 & $11.943 \pm 0.048$ & $ 26585.2\pm  1155.8$ \\
  715.0 & {\rm J}     &    7.8 & $11.990 \pm 0.048$ & $ 25473.0\pm  1107.9$ \\
  723.0 & {\rm J}     &    7.8 & $11.979 \pm 0.048$ & $ 25734.7\pm  1119.3$ \\
  743.0 & {\rm J}     &    7.8 & $12.104 \pm 0.048$ & $ 22940.3\pm   998.4$ \\
  751.3 & {\rm J}     &    7.8 & $12.121 \pm 0.048$ & $ 22573.5\pm   982.7$ \\
  759.2 & {\rm J}     &    7.8 & $12.146 \pm 0.048$ & $ 22069.9\pm   961.0$ \\
  779.3 & {\rm J}     &    7.8 & $12.166 \pm 0.048$ & $ 21657.1\pm   943.5$ \\
  787.5 & {\rm J}     &    7.8 & $12.135 \pm 0.048$ & $ 22282.3\pm   970.5$ \\
  795.5 & {\rm J}     &    7.8 & $12.172 \pm 0.048$ & $ 21531.8\pm   938.2$ \\
  815.5 & {\rm J}     &    7.8 & $12.257 \pm 0.048$ & $ 19919.6\pm   870.1$ \\
  823.8 & {\rm J}     &    7.8 & $12.277 \pm 0.048$ & $ 19547.0\pm   852.6$ \\
  831.7 & {\rm J}     &    7.8 & $12.249 \pm 0.048$ & $ 20066.9\pm   874.7$ \\
  851.7 & {\rm J}     &    7.8 & $12.345 \pm 0.048$ & $ 18363.7\pm   801.7$ \\
  860.0 & {\rm J}     &    7.8 & $12.363 \pm 0.048$ & $ 18058.4\pm   788.8$ \\
  867.9 & {\rm J}     &    7.8 & $12.384 \pm 0.048$ & $ 17719.0\pm   774.0$ \\
  888.0 & {\rm J}     &    7.8 & $12.394 \pm 0.048$ & $ 17548.5\pm   766.5$ \\
  896.2 & {\rm J}     &    7.8 & $12.465 \pm 0.049$ & $ 16451.3\pm   719.2$ \\
  904.1 & {\rm J}     &    7.8 & $12.449 \pm 0.049$ & $ 16683.2\pm   729.2$ \\
  924.1 & {\rm J}     &    7.8 & $12.502 \pm 0.049$ & $ 15886.9\pm   696.1$ \\
  932.4 & {\rm J}     &    7.8 & $12.500 \pm 0.049$ & $ 15920.6\pm   697.4$ \\
  940.3 & {\rm J}     &    7.8 & $12.500 \pm 0.049$ & $ 15929.4\pm   697.5$ \\
  960.3 & {\rm J}     &    7.8 & $12.616 \pm 0.049$ & $ 14310.0\pm   628.1$ \\
  968.5 & {\rm J}     &    7.8 & $12.575 \pm 0.049$ & $ 14866.2\pm   652.0$ \\
  976.5 & {\rm J}     &    7.8 & $12.541 \pm 0.049$ & $ 15327.8\pm   671.2$ \\
  996.5 & {\rm J}     &    7.8 & $12.655 \pm 0.049$ & $ 13798.7\pm   606.3$ \\
 1004.8 & {\rm J}     &    7.8 & $12.665 \pm 0.049$ & $ 13674.8\pm   601.5$ \\
 1012.7 & {\rm J}     &    7.8 & $12.673 \pm 0.049$ & $ 13574.4\pm   597.1$ \\
 1032.7 & {\rm J}     &    7.8 & $12.758 \pm 0.049$ & $ 12552.2\pm   552.9$ \\
 1041.0 & {\rm J}     &    7.8 & $12.854 \pm 0.049$ & $ 11491.0\pm   506.8$ \\
 1049.0 & {\rm J}     &    7.8 & $12.823 \pm 0.049$ & $ 11823.9\pm   522.1$ \\
 1069.0 & {\rm J}     &    7.8 & $12.905 \pm 0.049$ & $ 10969.8\pm   485.8$ \\
 1077.2 & {\rm J}     &    7.8 & $12.868 \pm 0.049$ & $ 11343.8\pm   502.8$ \\
 1085.2 & {\rm J}     &    7.8 & $12.853 \pm 0.049$ & $ 11500.6\pm   507.8$ \\
 1105.2 & {\rm J}     &    7.8 & $12.922 \pm 0.049$ & $ 10793.4\pm   479.0$ \\
 1113.5 & {\rm J}     &    7.8 & $12.938 \pm 0.049$ & $ 10633.6\pm   472.6$ \\
 1121.4 & {\rm J}     &    7.8 & $12.929 \pm 0.049$ & $ 10726.1\pm   475.6$ \\
 1141.4 & {\rm J}     &    7.8 & $13.035 \pm 0.050$ & $  9731.9\pm   437.5$ \\
 1149.7 & {\rm J}     &    7.8 & $13.048 \pm 0.050$ & $  9609.0\pm   429.3$ \\
 1157.6 & {\rm J}     &    7.8 & $13.041 \pm 0.049$ & $  9677.4\pm   430.5$ \\
 1177.6 & {\rm J}     &    7.8 & $12.998 \pm 0.049$ & $ 10067.5\pm   446.8$ \\
 1185.8 & {\rm J}     &    7.8 & $13.036 \pm 0.049$ & $  9714.9\pm   431.2$ \\
 1193.8 & {\rm J}     &    7.8 & $13.094 \pm 0.050$ & $  9216.4\pm   412.6$ \\
 1221.5 & {\rm J}     &   23.5 & $13.101 \pm 0.035$ & $  9150.4\pm   287.9$ \\
 1257.5 & {\rm J}     &   23.5 & $13.150 \pm 0.035$ & $  8748.2\pm   275.3$ \\
 1293.5 & {\rm J}     &   23.5 & $13.311 \pm 0.035$ & $  7545.4\pm   238.1$ \\
 1330.0 & {\rm J}     &   23.5 & $13.307 \pm 0.035$ & $  7573.9\pm   239.0$ \\
 1366.0 & {\rm J}     &   23.5 & $13.412 \pm 0.035$ & $  6871.9\pm   217.3$ \\
 1402.0 & {\rm J}     &   23.5 & $13.516 \pm 0.035$ & $  6244.8\pm   198.4$ \\
 1438.5 & {\rm J}     &   23.5 & $13.479 \pm 0.035$ & $  6465.5\pm   205.1$ \\
 1474.5 & {\rm J}     &   23.5 & $13.587 \pm 0.035$ & $  5847.9\pm   186.1$ \\
 1510.5 & {\rm J}     &   23.5 & $13.610 \pm 0.035$ & $  5729.0\pm   183.0$ \\
 1547.0 & {\rm J}     &   23.5 & $13.690 \pm 0.035$ & $  5321.1\pm   170.1$ \\
 1583.0 & {\rm J}     &   23.5 & $13.708 \pm 0.035$ & $  5232.1\pm   167.5$ \\
 1619.5 & {\rm J}     &   23.5 & $13.761 \pm 0.035$ & $  4982.9\pm   159.5$ \\
 1656.5 & {\rm J}     &   23.5 & $13.834 \pm 0.036$ & $  4658.9\pm   150.3$ \\
 1692.5 & {\rm J}     &   23.5 & $13.829 \pm 0.036$ & $  4682.5\pm   150.9$ \\
 1729.0 & {\rm J}     &   23.5 & $13.857 \pm 0.036$ & $  4564.2\pm   147.3$ \\
 1765.0 & {\rm J}     &   23.5 & $13.911 \pm 0.036$ & $  4341.9\pm   140.2$ \\
 1801.5 & {\rm J}     &   23.5 & $14.011 \pm 0.036$ & $  3959.5\pm   128.9$ \\
 1837.5 & {\rm J}     &   23.5 & $14.115 \pm 0.037$ & $  3598.5\pm   120.7$ \\
 1873.5 & {\rm J}     &   23.5 & $14.069 \pm 0.036$ & $  3752.5\pm   122.5$ \\
 1910.0 & {\rm J}     &   23.5 & $14.084 \pm 0.036$ & $  3701.0\pm   120.7$ \\
 1964.0 & {\rm J}     &   47.1 & $14.171 \pm 0.036$ & $  3417.3\pm   110.9$ \\
 2036.5 & {\rm J}     &   47.1 & $14.214 \pm 0.036$ & $  3282.8\pm   106.5$ \\
 2109.0 & {\rm J}     &   47.1 & $14.254 \pm 0.035$ & $  3165.2\pm   101.8$ \\
 2181.5 & {\rm J}     &   47.1 & $14.377 \pm 0.036$ & $  2827.2\pm    92.3$ \\
 2254.0 & {\rm J}     &   47.1 & $14.330 \pm 0.037$ & $  2951.8\pm    97.6$ \\
 2326.0 & {\rm J}     &   47.1 & $14.457 \pm 0.037$ & $  2625.7\pm    86.9$ \\
 2399.5 & {\rm J}     &   47.1 & $14.510 \pm 0.037$ & $  2500.3\pm    83.2$ \\
 2472.0 & {\rm J}     &   47.1 & $14.536 \pm 0.037$ & $  2441.0\pm    81.4$ \\
 2544.5 & {\rm J}     &   47.1 & $14.568 \pm 0.037$ & $  2369.2\pm    78.4$ \\
 2616.5 & {\rm J}     &   47.1 & $14.628 \pm 0.037$ & $  2242.0\pm    74.8$ \\
 2689.0 & {\rm J}     &   47.1 & $14.670 \pm 0.037$ & $  2156.8\pm    72.8$ \\
 2761.5 & {\rm J}     &   47.1 & $14.748 \pm 0.037$ & $  2008.7\pm    68.0$ \\
 2834.0 & {\rm J}     &   47.1 & $14.781 \pm 0.037$ & $  1947.5\pm    65.8$ \\
 2906.5 & {\rm J}     &   47.1 & $14.850 \pm 0.038$ & $  1827.9\pm    62.7$ \\
 2978.5 & {\rm J}     &   47.1 & $14.883 \pm 0.038$ & $  1773.7\pm    61.2$ \\
 3051.0 & {\rm J}     &   47.1 & $14.832 \pm 0.038$ & $  1858.3\pm    63.9$ \\
 3123.5 & {\rm J}     &   47.1 & $14.894 \pm 0.038$ & $  1756.0\pm    61.1$ \\
 3195.5 & {\rm J}     &   47.1 & $15.008 \pm 0.039$ & $  1579.9\pm    55.1$ \\
 3268.5 & {\rm J}     &   47.1 & $14.987 \pm 0.038$ & $  1611.7\pm    56.1$ \\
 3340.5 & {\rm J}     &   47.1 & $14.922 \pm 0.039$ & $  1710.8\pm    60.1$ \\
 3414.0 & {\rm J}     &   47.1 & $15.068 \pm 0.039$ & $  1495.4\pm    53.1$ \\
 3486.5 & {\rm J}     &   47.1 & $15.072 \pm 0.039$ & $  1489.9\pm    52.4$ \\
 3559.0 & {\rm J}     &   47.1 & $15.005 \pm 0.038$ & $  1585.5\pm    55.1$ \\
 3632.0 & {\rm J}     &   47.1 & $15.174 \pm 0.040$ & $  1356.7\pm    48.8$ \\
 3686.5 & {\rm J}     &   23.5 & $15.098 \pm 0.039$ & $  1455.2\pm    51.7$ \\
 3892.5 & {\rm J}     &  227.6 & $15.265 \pm 0.038$ & $  1247.7\pm    42.5$ \\
 4251.0 & {\rm J}     &  235.4 & $15.369 \pm 0.038$ & $  1133.2\pm    39.1$ \\
 4613.0 & {\rm J}     &  235.4 & $15.501 \pm 0.039$ & $  1003.6\pm    35.3$ \\
 4975.5 & {\rm J}     &  235.4 & $15.586 \pm 0.039$ & $   928.3\pm    32.7$ \\
 5338.5 & {\rm J}     &  235.4 & $15.748 \pm 0.041$ & $   799.2\pm    29.3$ \\
 5703.0 & {\rm J}     &  235.4 & $15.774 \pm 0.041$ & $   780.9\pm    29.0$ \\
 6068.5 & {\rm J}     &  235.4 & $15.870 \pm 0.043$ & $   714.8\pm    27.6$ \\
 6431.5 & {\rm J}     &  235.4 & $15.811 \pm 0.041$ & $   754.2\pm    28.0$ \\
 6860.0 & {\rm J}     &  313.9 & $16.019 \pm 0.042$ & $   622.9\pm    23.7$ \\
 7613.0 & {\rm J}     &  353.2 & $16.139 \pm 0.042$ & $   557.5\pm    21.3$ \\
 8248.0 & {\rm J}     &  470.9 & $16.236 \pm 0.042$ & $   509.9\pm    19.5$ \\
 8973.0 & {\rm J}     &  470.9 & $16.475 \pm 0.045$ & $   409.4\pm    16.7$ \\
 9698.5 & {\rm J}     &  470.9 & $16.469 \pm 0.051$ & $   411.4\pm    19.0$ \\
10424.0 & {\rm J}     &  470.9 & $16.649 \pm 0.047$ & $   348.7\pm    14.8$ \\
11738.5 & {\rm J}     & 1169.3 & $16.832 \pm 0.047$ & $   294.6\pm    12.5$ \\
13521.5 & {\rm J}     & 1138.0 & $16.962 \pm 0.049$ & $   261.2\pm    11.5$ \\
15328.5 & {\rm J}     & 1169.3 & $17.014 \pm 0.049$ & $   249.2\pm    11.1$ \\
17109.5 & {\rm J}     & 1138.0 & $17.307 \pm 0.057$ & $   190.3\pm     9.7$ \\
19132.5 & {\rm J}     & 1412.6 & $17.505 \pm 0.059$ & $   158.5\pm     8.4$ \\
21321.0 & {\rm J}     & 1294.9 & $17.528 \pm 0.060$ & $   155.2\pm     8.4$ \\
  344.0 & {\rm H}     &    7.8 & $ 9.639 \pm 0.042$ & $142696.2\pm  5421.2$ \\
  352.3 & {\rm H}     &    7.8 & $ 9.721 \pm 0.042$ & $132364.7\pm  5029.4$ \\
  360.2 & {\rm H}     &    7.8 & $ 9.753 \pm 0.042$ & $128513.3\pm  4883.6$ \\
  380.1 & {\rm H}     &    7.8 & $ 9.946 \pm 0.042$ & $107582.1\pm  4088.8$ \\
  388.4 & {\rm H}     &    7.8 & $ 9.985 \pm 0.042$ & $103750.1\pm  3944.2$ \\
  396.3 & {\rm H}     &    7.8 & $10.115 \pm 0.042$ & $ 92078.9\pm  3501.5$ \\
  416.3 & {\rm H}     &    7.8 & $10.127 \pm 0.042$ & $ 91066.8\pm  3464.2$ \\
  424.5 & {\rm H}     &    7.8 & $10.177 \pm 0.042$ & $ 86920.1\pm  3306.4$ \\
  432.4 & {\rm H}     &    7.8 & $10.245 \pm 0.042$ & $ 81665.8\pm  3107.6$ \\
  452.4 & {\rm H}     &    7.8 & $10.288 \pm 0.042$ & $ 78465.8\pm  2985.3$ \\
  460.7 & {\rm H}     &    7.8 & $10.352 \pm 0.042$ & $ 73981.1\pm  2815.2$ \\
  468.6 & {\rm H}     &    7.8 & $10.396 \pm 0.042$ & $ 71062.5\pm  2704.6$ \\
  488.6 & {\rm H}     &    7.8 & $10.545 \pm 0.042$ & $ 61944.1\pm  2359.9$ \\
  496.9 & {\rm H}     &    7.8 & $10.534 \pm 0.042$ & $ 62551.9\pm  2383.6$ \\
  504.8 & {\rm H}     &    7.8 & $10.607 \pm 0.042$ & $ 58516.7\pm  2230.2$ \\
  525.8 & {\rm H}     &    7.8 & $10.794 \pm 0.042$ & $ 49244.8\pm  1878.6$ \\
  534.1 & {\rm H}     &    7.8 & $10.822 \pm 0.042$ & $ 47991.1\pm  1832.7$ \\
  542.0 & {\rm H}     &    7.8 & $10.863 \pm 0.042$ & $ 46221.1\pm  1765.0$ \\
  561.9 & {\rm H}     &    7.8 & $10.892 \pm 0.042$ & $ 45002.9\pm  1718.1$ \\
  570.2 & {\rm H}     &    7.8 & $10.847 \pm 0.042$ & $ 46885.7\pm  1790.4$ \\
  578.2 & {\rm H}     &    7.8 & $10.914 \pm 0.042$ & $ 44108.3\pm  1684.4$ \\
  598.2 & {\rm H}     &    7.8 & $10.981 \pm 0.042$ & $ 41476.3\pm  1586.0$ \\
  606.4 & {\rm H}     &    7.8 & $11.009 \pm 0.042$ & $ 40383.2\pm  1545.1$ \\
  614.4 & {\rm H}     &    7.8 & $11.032 \pm 0.042$ & $ 39540.3\pm  1514.3$ \\
  634.4 & {\rm H}     &    7.8 & $11.073 \pm 0.042$ & $ 38096.1\pm  1457.2$ \\
  642.7 & {\rm H}     &    7.8 & $11.144 \pm 0.042$ & $ 35684.6\pm  1367.9$ \\
  650.6 & {\rm H}     &    7.8 & $11.145 \pm 0.042$ & $ 35632.0\pm  1364.2$ \\
  670.6 & {\rm H}     &    7.8 & $11.202 \pm 0.042$ & $ 33825.2\pm  1295.1$ \\
  678.9 & {\rm H}     &    7.8 & $11.309 \pm 0.043$ & $ 30656.3\pm  1177.7$ \\
  686.8 & {\rm H}     &    7.8 & $11.319 \pm 0.043$ & $ 30352.9\pm  1166.4$ \\
  706.8 & {\rm H}     &    7.8 & $11.316 \pm 0.043$ & $ 30442.5\pm  1169.0$ \\
  715.0 & {\rm H}     &    7.8 & $11.287 \pm 0.043$ & $ 31283.9\pm  1201.8$ \\
  723.0 & {\rm H}     &    7.8 & $11.328 \pm 0.043$ & $ 30105.1\pm  1156.5$ \\
  743.0 & {\rm H}     &    7.8 & $11.483 \pm 0.043$ & $ 26097.6\pm  1003.7$ \\
  751.3 & {\rm H}     &    7.8 & $11.498 \pm 0.043$ & $ 25744.3\pm   991.2$ \\
  759.2 & {\rm H}     &    7.8 & $11.481 \pm 0.043$ & $ 26150.5\pm  1009.3$ \\
  779.3 & {\rm H}     &    7.8 & $11.503 \pm 0.043$ & $ 25635.4\pm   989.0$ \\
  787.5 & {\rm H}     &    7.8 & $11.574 \pm 0.043$ & $ 24008.3\pm   928.3$ \\
  795.5 & {\rm H}     &    7.8 & $11.597 \pm 0.043$ & $ 23511.5\pm   910.3$ \\
  815.5 & {\rm H}     &    7.8 & $11.646 \pm 0.043$ & $ 22469.8\pm   876.0$ \\
  823.8 & {\rm H}     &    7.8 & $11.697 \pm 0.043$ & $ 21432.9\pm   830.2$ \\
  831.7 & {\rm H}     &    7.8 & $11.667 \pm 0.043$ & $ 22035.4\pm   856.0$ \\
  851.7 & {\rm H}     &    7.8 & $11.662 \pm 0.043$ & $ 22143.2\pm   858.5$ \\
  860.0 & {\rm H}     &    7.8 & $11.688 \pm 0.043$ & $ 21617.2\pm   837.3$ \\
  867.9 & {\rm H}     &    7.8 & $11.695 \pm 0.043$ & $ 21474.4\pm   834.2$ \\
  888.0 & {\rm H}     &    7.8 & $11.807 \pm 0.044$ & $ 19376.7\pm   761.3$ \\
  896.2 & {\rm H}     &    7.8 & $11.842 \pm 0.043$ & $ 18762.0\pm   729.2$ \\
  904.1 & {\rm H}     &    7.8 & $11.889 \pm 0.043$ & $ 17972.2\pm   697.4$ \\
  924.1 & {\rm H}     &    7.8 & $11.892 \pm 0.043$ & $ 17914.3\pm   701.0$ \\
  932.4 & {\rm H}     &    7.8 & $11.903 \pm 0.043$ & $ 17725.6\pm   694.8$ \\
  940.3 & {\rm H}     &    7.8 & $11.840 \pm 0.043$ & $ 18789.7\pm   735.7$ \\
  960.3 & {\rm H}     &    7.8 & $11.990 \pm 0.044$ & $ 16372.7\pm   645.6$ \\
  968.5 & {\rm H}     &    7.8 & $12.023 \pm 0.044$ & $ 15882.5\pm   627.1$ \\
  976.5 & {\rm H}     &    7.8 & $11.960 \pm 0.044$ & $ 16825.2\pm   661.5$ \\
  996.5 & {\rm H}     &    7.8 & $11.959 \pm 0.044$ & $ 16846.9\pm   669.9$ \\
 1004.8 & {\rm H}     &    7.8 & $12.030 \pm 0.044$ & $ 15774.7\pm   624.4$ \\
 1012.7 & {\rm H}     &    7.8 & $12.037 \pm 0.044$ & $ 15676.2\pm   621.3$ \\
 1032.7 & {\rm H}     &    7.8 & $12.130 \pm 0.044$ & $ 14381.4\pm   571.1$ \\
 1041.0 & {\rm H}     &    7.8 & $12.187 \pm 0.044$ & $ 13652.1\pm   544.7$ \\
 1049.0 & {\rm H}     &    7.8 & $12.172 \pm 0.044$ & $ 13842.0\pm   554.2$ \\
 1069.0 & {\rm H}     &    7.8 & $12.242 \pm 0.045$ & $ 12981.4\pm   522.4$ \\
 1077.2 & {\rm H}     &    7.8 & $12.228 \pm 0.045$ & $ 13145.0\pm   531.8$ \\
 1085.2 & {\rm H}     &    7.8 & $12.246 \pm 0.045$ & $ 12927.7\pm   521.4$ \\
 1105.2 & {\rm H}     &    7.8 & $12.249 \pm 0.045$ & $ 12895.6\pm   526.2$ \\
 1113.5 & {\rm H}     &    7.8 & $12.239 \pm 0.045$ & $ 13008.9\pm   530.9$ \\
 1121.4 & {\rm H}     &    7.8 & $12.323 \pm 0.045$ & $ 12039.3\pm   490.9$ \\
 1141.4 & {\rm H}     &    7.8 & $12.341 \pm 0.046$ & $ 11851.1\pm   493.9$ \\
 1149.7 & {\rm H}     &    7.8 & $12.417 \pm 0.046$ & $ 11049.9\pm   460.1$ \\
 1157.6 & {\rm H}     &    7.8 & $12.433 \pm 0.046$ & $ 10886.3\pm   447.2$ \\
 1177.6 & {\rm H}     &    7.8 & $12.370 \pm 0.045$ & $ 11535.6\pm   468.5$ \\
 1185.8 & {\rm H}     &    7.8 & $12.410 \pm 0.045$ & $ 11112.2\pm   454.9$ \\
 1193.8 & {\rm H}     &    7.8 & $12.467 \pm 0.047$ & $ 10553.6\pm   446.3$ \\
 1221.5 & {\rm H}     &   23.5 & $12.389 \pm 0.049$ & $ 11330.3\pm   495.5$ \\
 1257.5 & {\rm H}     &   23.5 & $12.508 \pm 0.049$ & $ 10156.9\pm   443.9$ \\
 1293.5 & {\rm H}     &   23.5 & $12.687 \pm 0.049$ & $  8613.1\pm   378.6$ \\
 1330.0 & {\rm H}     &   23.5 & $12.653 \pm 0.049$ & $  8885.5\pm   389.3$ \\
 1366.0 & {\rm H}     &   23.5 & $12.691 \pm 0.049$ & $  8584.6\pm   376.5$ \\
 1402.0 & {\rm H}     &   23.5 & $12.882 \pm 0.049$ & $  7196.5\pm   316.5$ \\
 1438.5 & {\rm H}     &   23.5 & $12.943 \pm 0.049$ & $  6805.2\pm   299.7$ \\
 1474.5 & {\rm H}     &   23.5 & $12.983 \pm 0.049$ & $  6557.2\pm   291.0$ \\
 1510.5 & {\rm H}     &   23.5 & $12.972 \pm 0.049$ & $  6624.0\pm   292.6$ \\
 1547.0 & {\rm H}     &   23.5 & $13.081 \pm 0.049$ & $  5991.8\pm   264.8$ \\
 1583.0 & {\rm H}     &   23.5 & $13.055 \pm 0.049$ & $  6138.2\pm   273.1$ \\
 1619.5 & {\rm H}     &   23.5 & $13.196 \pm 0.049$ & $  5391.6\pm   239.7$ \\
 1656.5 & {\rm H}     &   23.5 & $13.354 \pm 0.050$ & $  4659.7\pm   208.3$ \\
 1692.5 & {\rm H}     &   23.5 & $13.224 \pm 0.050$ & $  5251.9\pm   235.6$ \\
 1729.0 & {\rm H}     &   23.5 & $13.205 \pm 0.050$ & $  5345.2\pm   238.5$ \\
 1765.0 & {\rm H}     &   23.5 & $13.364 \pm 0.050$ & $  4617.4\pm   207.2$ \\
 1801.5 & {\rm H}     &   23.5 & $13.503 \pm 0.050$ & $  4064.1\pm   183.2$ \\
 1837.5 & {\rm H}     &   23.5 & $13.402 \pm 0.051$ & $  4459.8\pm   202.9$ \\
 1891.5 & {\rm H}     &   47.1 & $13.537 \pm 0.049$ & $  3937.7\pm   175.1$ \\
 1964.0 & {\rm H}     &   47.1 & $13.554 \pm 0.050$ & $  3874.7\pm   173.0$ \\
 2036.5 & {\rm H}     &   47.1 & $13.655 \pm 0.050$ & $  3533.5\pm   159.7$ \\
 2109.0 & {\rm H}     &   47.1 & $13.775 \pm 0.050$ & $  3163.2\pm   141.2$ \\
 2181.5 & {\rm H}     &   47.1 & $13.746 \pm 0.050$ & $  3248.5\pm   146.3$ \\
 2254.0 & {\rm H}     &   47.1 & $13.783 \pm 0.050$ & $  3139.9\pm   142.1$ \\
 2326.0 & {\rm H}     &   47.1 & $13.863 \pm 0.051$ & $  2915.5\pm   132.5$ \\
 2399.5 & {\rm H}     &   47.1 & $13.990 \pm 0.050$ & $  2594.7\pm   117.6$ \\
 2472.0 & {\rm H}     &   47.1 & $13.904 \pm 0.051$ & $  2808.0\pm   128.1$ \\
 2544.5 & {\rm H}     &   47.1 & $14.034 \pm 0.051$ & $  2491.2\pm   113.7$ \\
 2616.5 & {\rm H}     &   47.1 & $14.062 \pm 0.051$ & $  2428.0\pm   111.5$ \\
 2689.0 & {\rm H}     &   47.1 & $14.074 \pm 0.051$ & $  2401.9\pm   110.8$ \\
 2761.5 & {\rm H}     &   47.1 & $14.205 \pm 0.052$ & $  2127.2\pm    99.8$ \\
 2834.0 & {\rm H}     &   47.1 & $14.160 \pm 0.051$ & $  2218.4\pm   101.8$ \\
 2906.5 & {\rm H}     &   47.1 & $14.187 \pm 0.052$ & $  2163.9\pm   100.6$ \\
 2978.5 & {\rm H}     &   47.1 & $14.278 \pm 0.054$ & $  1989.6\pm    95.9$ \\
 3051.0 & {\rm H}     &   47.1 & $14.338 \pm 0.053$ & $  1883.5\pm    89.3$ \\
 3123.5 & {\rm H}     &   47.1 & $14.344 \pm 0.053$ & $  1873.1\pm    89.1$ \\
 3195.5 & {\rm H}     &   47.1 & $14.422 \pm 0.053$ & $  1742.0\pm    82.4$ \\
 3268.5 & {\rm H}     &   47.1 & $14.303 \pm 0.052$ & $  1945.0\pm    91.3$ \\
 3340.5 & {\rm H}     &   47.1 & $14.520 \pm 0.056$ & $  1592.5\pm    79.9$ \\
 3414.0 & {\rm H}     &   47.1 & $14.488 \pm 0.053$ & $  1640.3\pm    78.7$ \\
 3486.5 & {\rm H}     &   47.1 & $14.321 \pm 0.052$\tablenotemark{x} & $  1912.3\pm    89.6$\tablenotemark{x} \\
 3559.0 & {\rm H}     &   47.1 & $14.517 \pm 0.056$ & $  1596.9\pm    80.7$ \\
 3632.0 & {\rm H}     &   47.1 & $14.508 \pm 0.054$ & $  1610.2\pm    78.8$ \\
 3892.5 & {\rm H}     &  227.6 & $14.753 \pm 0.053$ & $  1284.6\pm    60.8$ \\
 4251.0 & {\rm H}     &  235.4 & $14.799 \pm 0.052$ & $  1232.0\pm    57.7$ \\
 4613.0 & {\rm H}     &  235.4 & $15.026 \pm 0.055$ & $   999.4\pm    49.3$ \\
 4975.5 & {\rm H}     &  235.4 & $15.101 \pm 0.055$ & $   932.2\pm    45.7$ \\
 5338.5 & {\rm H}     &  235.4 & $15.108 \pm 0.056$ & $   926.8\pm    46.4$ \\
 5703.0 & {\rm H}     &  235.4 & $15.129 \pm 0.055$ & $   908.8\pm    44.5$ \\
 6068.5 & {\rm H}     &  235.4 & $15.357 \pm 0.056$ & $   736.4\pm    37.2$ \\
 6431.5 & {\rm H}     &  235.4 & $15.497 \pm 0.055$ & $   647.4\pm    31.9$ \\
 6860.0 & {\rm H}     &  313.9 & $15.469 \pm 0.056$ & $   664.5\pm    33.6$ \\
 7613.0 & {\rm H}     &  353.2 & $15.662 \pm 0.058$ & $   556.3\pm    28.8$ \\
 8066.5 & {\rm H}     &  470.9 & $15.827 \pm 0.059$ & $   477.9\pm    25.1$ \\
 8973.0 & {\rm H}     &  470.9 & $15.915 \pm 0.060$ & $   440.4\pm    23.7$ \\
10061.5 & {\rm H}     &  894.7 & $16.059 \pm 0.059$ & $   385.8\pm    20.4$ \\
11738.5 & {\rm H}     & 1169.3 & $16.242 \pm 0.060$ & $   326.0\pm    17.6$ \\
13511.0 & {\rm H}     & 1106.6 & $16.278 \pm 0.061$ & $   315.3\pm    17.3$ \\
15328.5 & {\rm H}     & 1169.3 & $16.577 \pm 0.065$ & $   239.5\pm    14.0$ \\
17109.5 & {\rm H}     &  973.2 & $16.677 \pm 0.074$ & $   218.4\pm    14.4$ \\
19132.5 & {\rm H}     & 1389.1 & $16.763 \pm 0.072$ & $   201.7\pm    12.9$ \\
21321.0 & {\rm H}     & 1404.8 & $16.856 \pm 0.070$ & $   185.1\pm    11.6$ \\
  344.0 & {$\rm K_s$} &    7.8 & $ 9.067 \pm 0.058$\tablenotemark{x} & $157495.6\pm  8197.4$\tablenotemark{x} \\
  352.3 & {$\rm K_s$} &    7.8 & $ 9.308 \pm 0.058$\tablenotemark{x} & $126102.6\pm  6564.2$\tablenotemark{x} \\
  360.2 & {$\rm K_s$} &    7.8 & $ 9.207 \pm 0.058$\tablenotemark{x} & $138421.8\pm  7205.9$\tablenotemark{x} \\
  380.1 & {$\rm K_s$} &    7.8 & $ 9.312 \pm 0.058$ & $125650.6\pm  6541.1$ \\
  388.4 & {$\rm K_s$} &    7.8 & $ 9.310 \pm 0.058$ & $125949.5\pm  6557.6$ \\
  396.3 & {$\rm K_s$} &    7.8 & $ 9.419 \pm 0.058$ & $113840.4\pm  5927.9$ \\
  416.3 & {$\rm K_s$} &    7.8 & $ 9.508 \pm 0.058$ & $104946.6\pm  5465.3$ \\
  424.5 & {$\rm K_s$} &    7.8 & $ 9.546 \pm 0.058$ & $101331.5\pm  5277.5$ \\
  432.4 & {$\rm K_s$} &    7.8 & $ 9.638 \pm 0.058$ & $ 93031.2\pm  4845.6$ \\
  452.4 & {$\rm K_s$} &    7.8 & $ 9.800 \pm 0.058$ & $ 80131.7\pm  4175.7$ \\
  460.7 & {$\rm K_s$} &    7.8 & $ 9.882 \pm 0.058$ & $ 74348.6\pm  3874.4$ \\
  468.6 & {$\rm K_s$} &    7.8 & $ 9.906 \pm 0.058$ & $ 72710.4\pm  3789.8$ \\
  488.6 & {$\rm K_s$} &    7.8 & $10.029 \pm 0.058$ & $ 64947.2\pm  3386.3$ \\
  496.9 & {$\rm K_s$} &    7.8 & $10.115 \pm 0.058$ & $ 59973.6\pm  3126.9$ \\
  504.8 & {$\rm K_s$} &    7.8 & $10.129 \pm 0.058$ & $ 59232.5\pm  3088.6$ \\
  525.8 & {$\rm K_s$} &    7.8 & $10.072 \pm 0.058$ & $ 62408.0\pm  3254.7$ \\
  534.1 & {$\rm K_s$} &    7.8 & $10.235 \pm 0.058$ & $ 53708.1\pm  2802.0$ \\
  542.0 & {$\rm K_s$} &    7.8 & $10.240 \pm 0.058$ & $ 53436.8\pm  2788.6$ \\
  561.9 & {$\rm K_s$} &    7.8 & $10.312 \pm 0.058$ & $ 50026.5\pm  2612.4$ \\
  570.2 & {$\rm K_s$} &    7.8 & $10.377 \pm 0.058$ & $ 47115.1\pm  2460.4$ \\
  578.2 & {$\rm K_s$} &    7.8 & $10.502 \pm 0.058$ & $ 42010.7\pm  2195.2$ \\
  598.2 & {$\rm K_s$} &    7.8 & $10.398 \pm 0.058$ & $ 46238.1\pm  2416.5$ \\
  606.4 & {$\rm K_s$} &    7.8 & $10.492 \pm 0.058$ & $ 42399.5\pm  2214.8$ \\
  614.4 & {$\rm K_s$} &    7.8 & $10.488 \pm 0.058$ & $ 42540.3\pm  2222.9$ \\
  634.4 & {$\rm K_s$} &    7.8 & $10.603 \pm 0.058$ & $ 38257.8\pm  2000.8$ \\
  642.7 & {$\rm K_s$} &    7.8 & $10.562 \pm 0.058$ & $ 39737.5\pm  2082.1$ \\
  650.6 & {$\rm K_s$} &    7.8 & $10.561 \pm 0.058$ & $ 39763.1\pm  2079.5$ \\
  670.6 & {$\rm K_s$} &    7.8 & $10.728 \pm 0.058$ & $ 34109.9\pm  1785.5$ \\
  678.9 & {$\rm K_s$} &    7.8 & $10.753 \pm 0.059$ & $ 33327.3\pm  1750.4$ \\
  686.8 & {$\rm K_s$} &    7.8 & $10.687 \pm 0.058$ & $ 35416.0\pm  1856.8$ \\
  706.8 & {$\rm K_s$} &    7.8 & $10.797 \pm 0.058$ & $ 32018.4\pm  1679.0$ \\
  715.0 & {$\rm K_s$} &    7.8 & $10.749 \pm 0.059$ & $ 33456.5\pm  1756.8$ \\
  723.0 & {$\rm K_s$} &    7.8 & $10.826 \pm 0.059$ & $ 31163.1\pm  1634.9$ \\
  743.0 & {$\rm K_s$} &    7.8 & $10.830 \pm 0.059$ & $ 31031.3\pm  1630.2$ \\
  751.3 & {$\rm K_s$} &    7.8 & $10.916 \pm 0.059$ & $ 28689.3\pm  1508.2$ \\
  759.2 & {$\rm K_s$} &    7.8 & $10.844 \pm 0.059$ & $ 30653.5\pm  1608.5$ \\
  779.3 & {$\rm K_s$} &    7.8 & $10.751 \pm 0.059$\tablenotemark{x} & $ 33376.5\pm  1754.2$\tablenotemark{x} \\
  787.5 & {$\rm K_s$} &    7.8 & $10.971 \pm 0.059$ & $ 27274.7\pm  1436.1$ \\
  795.5 & {$\rm K_s$} &    7.8 & $11.003 \pm 0.059$ & $ 26475.3\pm  1392.5$ \\
  815.5 & {$\rm K_s$} &    7.8 & $10.949 \pm 0.059$ & $ 27827.9\pm  1469.6$ \\
  823.8 & {$\rm K_s$} &    7.8 & $11.160 \pm 0.059$ & $ 22915.0\pm  1207.5$ \\
  831.7 & {$\rm K_s$} &    7.8 & $11.169 \pm 0.059$ & $ 22721.7\pm  1198.6$ \\
  851.7 & {$\rm K_s$} &    7.8 & $11.092 \pm 0.059$ & $ 24391.6\pm  1288.9$ \\
  860.0 & {$\rm K_s$} &    7.8 & $11.106 \pm 0.059$ & $ 24070.2\pm  1269.7$ \\
  867.9 & {$\rm K_s$} &    7.8 & $11.130 \pm 0.059$ & $ 23544.0\pm  1243.4$ \\
  888.0 & {$\rm K_s$} &    7.8 & $11.089 \pm 0.059$ & $ 24450.1\pm  1288.7$ \\
  896.2 & {$\rm K_s$} &    7.8 & $11.157 \pm 0.059$ & $ 22963.6\pm  1212.0$ \\
  904.1 & {$\rm K_s$} &    7.8 & $11.225 \pm 0.059$ & $ 21575.5\pm  1138.8$ \\
  924.1 & {$\rm K_s$} &    7.8 & $11.267 \pm 0.059$ & $ 20756.8\pm  1100.9$ \\
  932.4 & {$\rm K_s$} &    7.8 & $11.319 \pm 0.059$ & $ 19784.3\pm  1047.6$ \\
  940.3 & {$\rm K_s$} &    7.8 & $11.288 \pm 0.059$ & $ 20359.2\pm  1079.1$ \\
  960.3 & {$\rm K_s$} &    7.8 & $11.337 \pm 0.059$ & $ 19455.4\pm  1031.2$ \\
  968.5 & {$\rm K_s$} &    7.8 & $11.367 \pm 0.059$ & $ 18932.2\pm  1009.3$ \\
  976.5 & {$\rm K_s$} &    7.8 & $11.377 \pm 0.059$ & $ 18751.7\pm   993.9$ \\
  996.5 & {$\rm K_s$} &    7.8 & $11.479 \pm 0.059$ & $ 17070.3\pm   909.7$ \\
 1004.8 & {$\rm K_s$} &    7.8 & $11.406 \pm 0.059$ & $ 18265.9\pm   971.1$ \\
 1012.7 & {$\rm K_s$} &    7.8 & $11.407 \pm 0.060$ & $ 18249.0\pm   973.2$ \\
 1032.7 & {$\rm K_s$} &    7.8 & $11.582 \pm 0.060$ & $ 15535.3\pm   830.4$ \\
 1041.0 & {$\rm K_s$} &    7.8 & $11.594 \pm 0.060$ & $ 15363.2\pm   826.1$ \\
 1049.0 & {$\rm K_s$} &    7.8 & $11.637 \pm 0.060$ & $ 14765.2\pm   794.9$ \\
 1069.0 & {$\rm K_s$} &    7.8 & $11.608 \pm 0.060$ & $ 15166.3\pm   821.2$ \\
 1077.2 & {$\rm K_s$} &    7.8 & $11.624 \pm 0.061$ & $ 14945.8\pm   811.5$ \\
 1085.2 & {$\rm K_s$} &    7.8 & $11.658 \pm 0.060$ & $ 14485.1\pm   783.6$ \\
 1105.2 & {$\rm K_s$} &    7.8 & $11.774 \pm 0.061$ & $ 13007.7\pm   705.6$ \\
 1113.5 & {$\rm K_s$} &    7.8 & $11.736 \pm 0.061$ & $ 13476.0\pm   733.4$ \\
 1121.4 & {$\rm K_s$} &    7.8 & $11.691 \pm 0.061$ & $ 14046.2\pm   762.6$ \\
 1141.4 & {$\rm K_s$} &    7.8 & $11.702 \pm 0.061$ & $ 13903.4\pm   762.7$ \\
 1149.7 & {$\rm K_s$} &    7.8 & $11.814 \pm 0.062$ & $ 12546.4\pm   691.5$ \\
 1157.6 & {$\rm K_s$} &    7.8 & $11.780 \pm 0.061$ & $ 12944.3\pm   702.5$ \\
 1177.6 & {$\rm K_s$} &    7.8 & $11.866 \pm 0.061$ & $ 11953.1\pm   656.0$ \\
 1185.8 & {$\rm K_s$} &    7.8 & $11.845 \pm 0.061$ & $ 12186.5\pm   669.9$ \\
 1193.8 & {$\rm K_s$} &    7.8 & $11.751 \pm 0.061$ & $ 13294.7\pm   729.7$ \\
 1221.5 & {$\rm K_s$} &   23.5 & $11.773 \pm 0.041$ & $ 13026.9\pm   480.1$ \\
 1257.5 & {$\rm K_s$} &   23.5 & $11.837 \pm 0.041$ & $ 12275.5\pm   452.2$ \\
 1293.5 & {$\rm K_s$} &   23.5 & $12.062 \pm 0.041$ & $  9985.3\pm   369.3$ \\
 1330.0 & {$\rm K_s$} &   23.5 & $12.046 \pm 0.041$ & $ 10130.7\pm   375.2$ \\
 1366.0 & {$\rm K_s$} &   23.5 & $12.123 \pm 0.041$ & $  9439.7\pm   351.0$ \\
 1402.0 & {$\rm K_s$} &   23.5 & $12.183 \pm 0.041$ & $  8927.3\pm   331.4$ \\
 1438.5 & {$\rm K_s$} &   23.5 & $12.227 \pm 0.041$ & $  8574.3\pm   321.2$ \\
 1474.5 & {$\rm K_s$} &   23.5 & $12.318 \pm 0.041$ & $  7883.5\pm   294.5$ \\
 1510.5 & {$\rm K_s$} &   23.5 & $12.382 \pm 0.042$ & $  7436.4\pm   279.9$ \\
 1583.0 & {$\rm K_s$} &   23.5 & $12.469 \pm 0.042$ & $  6859.9\pm   258.8$ \\
 1619.5 & {$\rm K_s$} &   23.5 & $12.590 \pm 0.042$ & $  6139.9\pm   233.5$ \\
 1656.5 & {$\rm K_s$} &   23.5 & $12.673 \pm 0.042$ & $  5684.3\pm   217.8$ \\
 1692.5 & {$\rm K_s$} &   23.5 & $12.594 \pm 0.043$ & $  6115.6\pm   235.4$ \\
 1729.0 & {$\rm K_s$} &   23.5 & $12.653 \pm 0.042$ & $  5790.0\pm   221.0$ \\
 1765.0 & {$\rm K_s$} &   23.5 & $12.728 \pm 0.043$ & $  5406.5\pm   209.8$ \\
 1801.5 & {$\rm K_s$} &   23.5 & $12.824 \pm 0.043$ & $  4948.1\pm   192.0$ \\
 1837.5 & {$\rm K_s$} &   23.5 & $12.654 \pm 0.044$\tablenotemark{x} & $  5787.4\pm   228.7$\tablenotemark{x} \\
 1891.5 & {$\rm K_s$} &   47.1 & $12.840 \pm 0.042$ & $  4876.6\pm   186.0$ \\
 1964.0 & {$\rm K_s$} &   47.1 & $12.915 \pm 0.042$ & $  4551.6\pm   173.3$ \\
 2036.5 & {$\rm K_s$} &   47.1 & $13.024 \pm 0.043$ & $  4117.2\pm   158.7$ \\
 2109.0 & {$\rm K_s$} &   47.1 & $13.147 \pm 0.042$ & $  3675.2\pm   140.9$ \\
 2181.5 & {$\rm K_s$} &   47.1 & $13.203 \pm 0.043$ & $  3489.8\pm   135.9$ \\
 2254.0 & {$\rm K_s$} &   47.1 & $13.267 \pm 0.044$ & $  3290.0\pm   130.9$ \\
 2326.0 & {$\rm K_s$} &   47.1 & $13.238 \pm 0.044$ & $  3380.0\pm   132.9$ \\
 2399.5 & {$\rm K_s$} &   47.1 & $13.334 \pm 0.044$ & $  3092.6\pm   123.7$ \\
 2472.0 & {$\rm K_s$} &   47.1 & $13.388 \pm 0.045$ & $  2942.3\pm   118.5$ \\
 2544.5 & {$\rm K_s$} &   47.1 & $13.490 \pm 0.045$ & $  2679.2\pm   107.8$ \\
 2616.5 & {$\rm K_s$} &   47.1 & $13.430 \pm 0.045$ & $  2830.6\pm   114.2$ \\
 2689.0 & {$\rm K_s$} &   47.1 & $13.455 \pm 0.045$ & $  2766.7\pm   111.9$ \\
 2761.5 & {$\rm K_s$} &   47.1 & $13.520 \pm 0.045$ & $  2606.2\pm   106.9$ \\
 2834.0 & {$\rm K_s$} &   47.1 & $13.650 \pm 0.046$ & $  2311.6\pm    96.7$ \\
 2906.5 & {$\rm K_s$} &   47.1 & $13.707 \pm 0.047$ & $  2194.8\pm    92.5$ \\
 2978.5 & {$\rm K_s$} &   47.1 & $13.861 \pm 0.048$ & $  1904.1\pm    82.7$ \\
 3051.0 & {$\rm K_s$} &   47.1 & $13.777 \pm 0.050$ & $  2056.7\pm    92.3$ \\
 3123.5 & {$\rm K_s$} &   47.1 & $13.813 \pm 0.049$ & $  1990.3\pm    87.9$ \\
 3195.5 & {$\rm K_s$} &   47.1 & $13.791 \pm 0.048$ & $  2030.3\pm    88.5$ \\
 3268.5 & {$\rm K_s$} &   47.1 & $13.905 \pm 0.052$ & $  1827.9\pm    84.9$ \\
 3340.5 & {$\rm K_s$} &   47.1 & $13.752 \pm 0.047$ & $  2104.6\pm    90.0$ \\
 3414.0 & {$\rm K_s$} &   47.1 & $13.816 \pm 0.048$ & $  1983.4\pm    85.5$ \\
 3486.5 & {$\rm K_s$} &   47.1 & $13.930 \pm 0.048$ & $  1786.3\pm    77.2$ \\
 3632.0 & {$\rm K_s$} &   47.1 & $14.083 \pm 0.056$ & $  1551.8\pm    77.9$ \\
 3892.5 & {$\rm K_s$} &  227.6 & $14.216 \pm 0.046$ & $  1373.3\pm    57.3$ \\
 4251.0 & {$\rm K_s$} &  235.4 & $14.376 \pm 0.047$ & $  1185.1\pm    50.1$ \\
 4613.0 & {$\rm K_s$} &  235.4 & $14.509 \pm 0.049$ & $  1048.3\pm    46.6$ \\
 4975.5 & {$\rm K_s$} &  235.4 & $14.562 \pm 0.049$ & $   997.9\pm    43.7$ \\
 5338.5 & {$\rm K_s$} &  235.4 & $14.846 \pm 0.053$\tablenotemark{x} & $   768.7\pm    36.5$\tablenotemark{x} \\
 5703.0 & {$\rm K_s$} &  235.4 & $14.653 \pm 0.050$ & $   917.8\pm    41.4$ \\
 6068.5 & {$\rm K_s$} &  235.4 & $14.835 \pm 0.055$ & $   776.2\pm    38.6$ \\
 6431.5 & {$\rm K_s$} &  235.4 & $14.854 \pm 0.052$ & $   762.7\pm    35.7$ \\
 6860.0 & {$\rm K_s$} &  313.9 & $14.989 \pm 0.053$ & $   673.5\pm    32.1$ \\
 7559.0 & {$\rm K_s$} &  423.8 & $15.173 \pm 0.053$ & $   568.6\pm    27.3$ \\
 8284.5 & {$\rm K_s$} &  376.7 & $15.394 \pm 0.064$ & $   463.9\pm    26.7$ \\
 8973.0 & {$\rm K_s$} &  470.9 & $15.357 \pm 0.055$ & $   480.0\pm    23.8$ \\
 9771.0 & {$\rm K_s$} &  282.5 & $15.335 \pm 0.071$ & $   490.0\pm    31.0$ \\
10424.0 & {$\rm K_s$} &  470.9 & $15.504 \pm 0.062$ & $   419.1\pm    23.2$ \\
11738.5 & {$\rm K_s$} & 1169.3 & $15.708 \pm 0.057$ & $   347.5\pm    17.7$ \\
13521.5 & {$\rm K_s$} & 1138.0 & $15.874 \pm 0.068$ & $   298.1\pm    18.1$ \\
15328.5 & {$\rm K_s$} & 1169.3 & $16.143 \pm 0.066$ & $   232.6\pm    13.7$ \\
17104.0 & {$\rm K_s$} &  753.4 & $16.146 \pm 0.079$ & $   232.1\pm    16.2$ \\
19096.0 & {$\rm K_s$} &  965.3 & $16.399 \pm 0.098$ & $   183.8\pm    15.8$ \\
21321.0 & {$\rm K_s$} & 1404.8 & $16.491 \pm 0.094$ & $   168.8\pm    14.0$ \\
\enddata 
\tablecomments{Includes only non-saturated exposures; photometry from the saturated epochs is given in Tables \ref{tab:shortr} and \ref{tab:annulus}}
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}

\begin{deluxetable}{lccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Short-Read Observations of GRB\,080319B During Saturated Regime \label{tab:shortr}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
   59.3 & {\rm J}     &  0.051 & $ 5.206 \pm 0.055$ & $1.32\times 10^{7}\pm6.52\times 10^{5}$ \\
   67.3 & {\rm J}     &  0.051 & $ 5.627 \pm 0.055$ & $8.94\times 10^{6}\pm4.43\times 10^{5}$ \\
   87.3 & {\rm J}     &  0.051 & $ 6.470 \pm 0.055$ & $4.11\times 10^{6}\pm2.04\times 10^{5}$ \\
   95.5 & {\rm J}     &  0.051 & $ 6.847 \pm 0.056$ & $2.91\times 10^{6}\pm1.45\times 10^{5}$ \\
  103.5 & {\rm J}     &  0.051 & $ 6.954 \pm 0.056$ & $2.63\times 10^{6}\pm1.32\times 10^{5}$ \\
  123.1 & {\rm J}     &  0.051 & $ 7.414 \pm 0.056$ & $1.72\times 10^{6}\pm8.71\times 10^{4}$ \\
  131.3 & {\rm J}     &  0.051 & $ 7.598 \pm 0.057$ & $1.45\times 10^{6}\pm7.39\times 10^{4}$ \\
  139.3 & {\rm J}     &  0.051 & $ 7.684 \pm 0.057$ & $1.34\times 10^{6}\pm6.84\times 10^{4}$ \\
  159.2 & {\rm J}     &  0.051 & $ 8.025 \pm 0.058$ & $981882.9\pm 51315.0$ \\
  167.5 & {\rm J}     &  0.051 & $ 8.142 \pm 0.059$ & $881534.9\pm 46414.5$ \\
  175.4 & {\rm J}     &  0.051 & $ 8.204 \pm 0.059$ & $832583.5\pm 44252.7$ \\
  195.4 & {\rm J}     &  0.051 & $ 8.572 \pm 0.062$ & $593072.1\pm 32968.8$ \\
  203.6 & {\rm J}     &  0.051 & $ 8.535 \pm 0.062$ & $613541.2\pm 33941.9$ \\
  211.6 & {\rm J}     &  0.051 & $ 8.680 \pm 0.065$ & $536917.4\pm 31222.2$ \\
  231.5 & {\rm J}     &  0.051 & $ 9.019 \pm 0.069$ & $392857.8\pm 24024.1$ \\
  239.8 & {\rm J}     &  0.051 & $ 9.192 \pm 0.071$ & $335233.7\pm 21205.8$ \\
  247.7 & {\rm J}     &  0.051 & $ 9.187 \pm 0.074$ & $336681.9\pm 22102.9$ \\
  267.7 & {\rm J}     &  0.051 & $ 9.514 \pm 0.082$ & $249103.6\pm 18037.5$ \\
  276.0 & {\rm J}     &  0.051 & $ 9.446 \pm 0.078$ & $265220.9\pm 18439.8$ \\
  283.9 & {\rm J}     &  0.051 & $ 9.606 \pm 0.089$ & $228974.9\pm 17981.3$ \\
   59.3 & {\rm H}     &  0.051 & $ 4.520 \pm 0.052$ & $1.59\times 10^{7}\pm7.47\times 10^{5}$ \\
   67.3 & {\rm H}     &  0.051 & $ 4.853 \pm 0.052$ & $1.17\times 10^{7}\pm5.50\times 10^{5}$ \\
   87.3 & {\rm H}     &  0.051 & $ 5.713 \pm 0.052$ & $5.30\times 10^{6}\pm2.50\times 10^{5}$ \\
   95.5 & {\rm H}     &  0.051 & $ 6.101 \pm 0.052$ & $3.71\times 10^{6}\pm1.75\times 10^{5}$ \\
  103.5 & {\rm H}     &  0.051 & $ 6.225 \pm 0.052$ & $3.31\times 10^{6}\pm1.56\times 10^{5}$ \\
  123.1 & {\rm H}     &  0.051 & $ 6.498 \pm 0.053$ & $2.58\times 10^{6}\pm1.22\times 10^{5}$ \\
  131.3 & {\rm H}     &  0.051 & $ 6.818 \pm 0.053$ & $1.92\times 10^{6}\pm9.14\times 10^{4}$ \\
  139.3 & {\rm H}     &  0.051 & $ 6.826 \pm 0.053$ & $1.90\times 10^{6}\pm9.07\times 10^{4}$ \\
  159.2 & {\rm H}     &  0.051 & $ 7.195 \pm 0.054$ & $1.36\times 10^{6}\pm6.60\times 10^{4}$ \\
  167.5 & {\rm H}     &  0.051 & $ 7.442 \pm 0.054$ & $1.08\times 10^{6}\pm5.27\times 10^{4}$ \\
  175.4 & {\rm H}     &  0.051 & $ 7.472 \pm 0.054$ & $1.05\times 10^{6}\pm5.12\times 10^{4}$ \\
  195.4 & {\rm H}     &  0.051 & $ 7.702 \pm 0.056$ & $849486.1\pm 42632.9$ \\
  203.6 & {\rm H}     &  0.051 & $ 7.794 \pm 0.056$ & $780635.8\pm 39444.5$ \\
  211.6 & {\rm H}     &  0.051 & $ 7.923 \pm 0.057$ & $693005.1\pm 35492.6$ \\
  231.5 & {\rm H}     &  0.051 & $ 8.009 \pm 0.058$ & $640537.1\pm 33515.6$ \\
  239.8 & {\rm H}     &  0.051 & $ 8.257 \pm 0.060$ & $509772.0\pm 27563.2$ \\
  247.7 & {\rm H}     &  0.051 & $ 8.394 \pm 0.063$ & $449113.5\pm 25494.0$ \\
  267.7 & {\rm H}     &  0.051 & $ 8.521 \pm 0.064$ & $399558.3\pm 22896.5$ \\
  276.0 & {\rm H}     &  0.051 & $ 8.620 \pm 0.065$ & $364676.9\pm 21241.0$ \\
  283.9 & {\rm H}     &  0.051 & $ 8.724 \pm 0.070$ & $331503.6\pm 20562.2$ \\
  303.9 & {\rm H}     &  0.051 & $ 8.923 \pm 0.078$ & $275996.9\pm 19061.8$ \\
  312.1 & {\rm H}     &  0.051 & $ 8.867 \pm 0.077$ & $290557.5\pm 20013.1$ \\
  320.1 & {\rm H}     &  0.051 & $ 9.120 \pm 0.085$ & $230182.6\pm 17264.2$ \\
   67.3 & {$\rm K_s$} &  0.051 & $ 4.362 \pm 0.048$ & $1.20\times 10^{7}\pm5.20\times 10^{5}$ \\
   87.3 & {$\rm K_s$} &  0.051 & $ 5.192 \pm 0.048$ & $5.59\times 10^{6}\pm2.43\times 10^{5}$ \\
   95.5 & {$\rm K_s$} &  0.051 & $ 5.308 \pm 0.048$ & $5.02\times 10^{6}\pm2.18\times 10^{5}$ \\
  103.5 & {$\rm K_s$} &  0.051 & $ 5.675 \pm 0.048$ & $3.58\times 10^{6}\pm1.56\times 10^{5}$ \\
  123.1 & {$\rm K_s$} &  0.051 & $ 5.922 \pm 0.049$ & $2.85\times 10^{6}\pm1.25\times 10^{5}$ \\
  131.3 & {$\rm K_s$} &  0.051 & $ 6.176 \pm 0.049$ & $2.26\times 10^{6}\pm9.93\times 10^{4}$ \\
  139.3 & {$\rm K_s$} &  0.051 & $ 6.226 \pm 0.049$ & $2.16\times 10^{6}\pm9.49\times 10^{4}$ \\
  159.2 & {$\rm K_s$} &  0.051 & $ 6.575 \pm 0.049$ & $1.56\times 10^{6}\pm6.95\times 10^{4}$ \\
  167.5 & {$\rm K_s$} &  0.051 & $ 6.651 \pm 0.050$ & $1.46\times 10^{6}\pm6.50\times 10^{4}$ \\
  175.4 & {$\rm K_s$} &  0.051 & $ 6.687 \pm 0.050$ & $1.41\times 10^{6}\pm6.30\times 10^{4}$ \\
  195.4 & {$\rm K_s$} &  0.051 & $ 7.016 \pm 0.051$ & $1.04\times 10^{6}\pm4.75\times 10^{4}$ \\
  203.6 & {$\rm K_s$} &  0.051 & $ 7.205 \pm 0.052$ & $874887.6\pm 40602.0$ \\
  211.6 & {$\rm K_s$} &  0.051 & $ 7.271 \pm 0.052$ & $823531.9\pm 38536.8$ \\
  231.5 & {$\rm K_s$} &  0.051 & $ 7.520 \pm 0.054$ & $654763.4\pm 31777.9$ \\
  239.8 & {$\rm K_s$} &  0.051 & $ 7.534 \pm 0.054$ & $646285.4\pm 31450.1$ \\
  247.7 & {$\rm K_s$} &  0.051 & $ 7.680 \pm 0.056$ & $564843.8\pm 28190.4$ \\
  267.7 & {$\rm K_s$} &  0.051 & $ 7.897 \pm 0.059$ & $462504.9\pm 24422.0$ \\
  276.0 & {$\rm K_s$} &  0.051 & $ 7.889 \pm 0.059$ & $466204.2\pm 24527.2$ \\
  283.9 & {$\rm K_s$} &  0.051 & $ 8.046 \pm 0.062$ & $403426.5\pm 22357.4$ \\
  303.9 & {$\rm K_s$} &  0.051 & $ 8.411 \pm 0.072$ & $288148.4\pm 18459.6$ \\
  312.1 & {$\rm K_s$} &  0.051 & $ 8.452 \pm 0.073$ & $277575.0\pm 18091.5$ \\
  320.1 & {$\rm K_s$} &  0.051 & $ 8.376 \pm 0.071$ & $297572.2\pm 18774.2$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UT 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{No saturated values were used in modeling.}
\end{deluxetable}

\begin{deluxetable}{lccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Annulus Photometry of GRB\,080319B During Saturated Regime\label{tab:annulus}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
   55.0 & {\rm J}     &    7.8 & $ 4.595 \pm 0.133$ & $2.31\times 10^{7}\pm2.66\times 10^{6}$ \\
   63.2 & {\rm J}     &    7.8 & $ 5.070 \pm 0.133$ & $1.49\times 10^{7}\pm1.72\times 10^{6}$ \\
   71.2 & {\rm J}     &    7.8 & $ 5.560 \pm 0.133$ & $9.51\times 10^{6}\pm1.10\times 10^{6}$ \\
   91.2 & {\rm J}     &    7.8 & $ 6.572 \pm 0.133$ & $3.74\times 10^{6}\pm4.31\times 10^{5}$ \\
   99.4 & {\rm J}     &    7.8 & $ 6.710 \pm 0.133$ & $3.30\times 10^{6}\pm3.80\times 10^{5}$ \\
  107.4 & {\rm J}     &    7.8 & $ 7.004 \pm 0.133$ & $2.51\times 10^{6}\pm2.90\times 10^{5}$ \\
  127.0 & {\rm J}     &    7.8 & $ 7.421 \pm 0.133$ & $1.71\times 10^{6}\pm1.97\times 10^{5}$ \\
  135.2 & {\rm J}     &    7.8 & $ 7.599 \pm 0.133$ & $1.45\times 10^{6}\pm1.67\times 10^{5}$ \\
  143.2 & {\rm J}     &    7.8 & $ 7.832 \pm 0.133$ & $1.17\times 10^{6}\pm1.35\times 10^{5}$ \\
  163.1 & {\rm J}     &    7.8 & $ 7.951 \pm 0.133$ & $1.05\times 10^{6}\pm1.21\times 10^{5}$ \\
  171.4 & {\rm J}     &    7.8 & $ 8.173 \pm 0.133$ & $856350.4\pm 98663.3$ \\
  179.3 & {\rm J}     &    7.8 & $ 8.436 \pm 0.133$ & $672288.4\pm 77456.8$ \\
  199.3 & {\rm J}     &    7.8 & $ 8.783 \pm 0.133$ & $488202.0\pm 56247.6$ \\
  207.5 & {\rm J}     &    7.8 & $ 8.824 \pm 0.133$ & $470395.8\pm 54196.1$ \\
  215.5 & {\rm J}     &    7.8 & $ 8.904 \pm 0.133$ & $436930.0\pm 50340.3$ \\
  235.4 & {\rm J}     &    7.8 & $ 9.090 \pm 0.133$ & $368067.5\pm 42406.4$ \\
  243.7 & {\rm J}     &    7.8 & $ 9.250 \pm 0.133$ & $317602.2\pm 36592.2$ \\
  251.6 & {\rm J}     &    7.8 & $ 9.267 \pm 0.133$ & $312633.6\pm 36019.7$ \\
  271.6 & {\rm J}     &    7.8 & $ 9.683 \pm 0.133$ & $213241.5\pm 24568.3$ \\
  279.9 & {\rm J}     &    7.8 & $ 9.808 \pm 0.133$ & $189946.7\pm 21884.5$ \\
  287.8 & {\rm J}     &    7.8 & $ 9.814 \pm 0.133$ & $189007.8\pm 21776.3$ \\
   55.0 & {\rm H}     &    7.8 & $ 4.387 \pm 0.191$ & $1.80\times 10^{7}\pm2.90\times 10^{6}$ \\
   63.2 & {\rm H}     &    7.8 & $ 4.805 \pm 0.191$ & $1.22\times 10^{7}\pm1.97\times 10^{6}$ \\
   71.2 & {\rm H}     &    7.8 & $ 5.159 \pm 0.191$ & $8.84\times 10^{6}\pm1.42\times 10^{6}$ \\
   91.2 & {\rm H}     &    7.8 & $ 5.818 \pm 0.191$ & $4.82\times 10^{6}\pm7.76\times 10^{5}$ \\
   99.4 & {\rm H}     &    7.8 & $ 6.386 \pm 0.191$ & $2.86\times 10^{6}\pm4.60\times 10^{5}$ \\
  107.4 & {\rm H}     &    7.8 & $ 6.421 \pm 0.191$ & $2.76\times 10^{6}\pm4.45\times 10^{5}$ \\
  127.0 & {\rm H}     &    7.8 & $ 6.756 \pm 0.191$ & $2.03\times 10^{6}\pm3.27\times 10^{5}$ \\
  135.2 & {\rm H}     &    7.8 & $ 7.040 \pm 0.191$ & $1.56\times 10^{6}\pm2.52\times 10^{5}$ \\
  143.2 & {\rm H}     &    7.8 & $ 7.048 \pm 0.191$ & $1.55\times 10^{6}\pm2.50\times 10^{5}$ \\
  163.1 & {\rm H}     &    7.8 & $ 7.476 \pm 0.191$ & $1.05\times 10^{6}\pm1.69\times 10^{5}$ \\
  171.4 & {\rm H}     &    7.8 & $ 7.461 \pm 0.191$ & $1.06\times 10^{6}\pm1.71\times 10^{5}$ \\
  179.3 & {\rm H}     &    7.8 & $ 7.624 \pm 0.191$ & $912709.1\pm147018.7$ \\
  199.3 & {\rm H}     &    7.8 & $ 8.025 \pm 0.191$ & $630888.4\pm101622.6$ \\
  207.5 & {\rm H}     &    7.8 & $ 8.130 \pm 0.191$ & $572965.1\pm 92292.4$ \\
  215.5 & {\rm H}     &    7.8 & $ 8.225 \pm 0.191$ & $524991.6\pm 84565.3$ \\
  235.4 & {\rm H}     &    7.8 & $ 8.364 \pm 0.191$ & $461849.2\pm 74396.1$ \\
  243.7 & {\rm H}     &    7.8 & $ 8.475 \pm 0.191$ & $416877.1\pm 67150.7$ \\
  251.6 & {\rm H}     &    7.8 & $ 8.549 \pm 0.191$ & $389235.4\pm 62700.0$ \\
  271.6 & {\rm H}     &    7.8 & $ 8.966 \pm 0.191$ & $265106.5\pm 42704.7$ \\
  279.9 & {\rm H}     &    7.8 & $ 9.138 \pm 0.191$ & $226458.2\pm 36479.4$ \\
  287.8 & {\rm H}     &    7.8 & $ 9.000 \pm 0.191$ & $257063.5\pm 41409.5$ \\
  307.8 & {\rm H}     &    7.8 & $ 8.990 \pm 0.191$ & $259305.8\pm 41771.9$ \\
  316.0 & {\rm H}     &    7.8 & $ 9.023 \pm 0.191$ & $251603.3\pm 40530.9$ \\
  324.0 & {\rm H}     &    7.8 & $ 9.458 \pm 0.191$ & $168531.2\pm 27149.7$ \\
   55.0 & {$\rm K_s$} &    7.8 & $ 3.853 \pm 0.463$ & $1.92\times 10^{7}\pm6.65\times 10^{6}$ \\
   63.2 & {$\rm K_s$} &    7.8 & $ 4.200 \pm 0.463$ & $1.39\times 10^{7}\pm4.83\times 10^{6}$ \\
   71.2 & {$\rm K_s$} &    7.8 & $ 4.510 \pm 0.463$ & $1.05\times 10^{7}\pm3.63\times 10^{6}$ \\
   91.2 & {$\rm K_s$} &    7.8 & $ 5.130 \pm 0.463$ & $5.91\times 10^{6}\pm2.05\times 10^{6}$ \\
   99.4 & {$\rm K_s$} &    7.8 & $ 5.659 \pm 0.463$ & $3.63\times 10^{6}\pm1.26\times 10^{6}$ \\
  107.4 & {$\rm K_s$} &    7.8 & $ 5.812 \pm 0.463$ & $3.16\times 10^{6}\pm1.09\times 10^{6}$ \\
  127.0 & {$\rm K_s$} &    7.8 & $ 6.105 \pm 0.463$ & $2.41\times 10^{6}\pm8.36\times 10^{5}$ \\
  135.2 & {$\rm K_s$} &    7.8 & $ 6.316 \pm 0.463$ & $1.98\times 10^{6}\pm6.88\times 10^{5}$ \\
  143.2 & {$\rm K_s$} &    7.8 & $ 6.506 \pm 0.463$ & $1.67\times 10^{6}\pm5.78\times 10^{5}$ \\
  163.1 & {$\rm K_s$} &    7.8 & $ 6.688 \pm 0.463$ & $1.41\times 10^{6}\pm4.89\times 10^{5}$ \\
  171.4 & {$\rm K_s$} &    7.8 & $ 6.861 \pm 0.463$ & $1.20\times 10^{6}\pm4.17\times 10^{5}$ \\
  179.3 & {$\rm K_s$} &    7.8 & $ 7.068 \pm 0.463$ & $992239.2\pm344242.9$ \\
  199.3 & {$\rm K_s$} &    7.8 & $ 7.345 \pm 0.463$ & $768890.1\pm266755.1$ \\
  207.5 & {$\rm K_s$} &    7.8 & $ 7.437 \pm 0.463$ & $706747.2\pm245195.6$ \\
  215.5 & {$\rm K_s$} &    7.8 & $ 7.577 \pm 0.463$ & $621144.1\pm215496.8$ \\
  235.4 & {$\rm K_s$} &    7.8 & $ 7.739 \pm 0.463$ & $535264.1\pm185702.0$ \\
  243.7 & {$\rm K_s$} &    7.8 & $ 7.883 \pm 0.463$ & $468516.0\pm162545.1$ \\
  251.6 & {$\rm K_s$} &    7.8 & $ 7.813 \pm 0.463$ & $499952.1\pm173451.0$ \\
  271.6 & {$\rm K_s$} &    7.8 & $ 8.373 \pm 0.463$ & $298274.8\pm103482.3$ \\
  279.9 & {$\rm K_s$} &    7.8 & $ 8.468 \pm 0.463$ & $273280.3\pm 94810.8$ \\
  287.8 & {$\rm K_s$} &    7.8 & $ 8.409 \pm 0.463$ & $288740.9\pm100174.4$ \\
  307.8 & {$\rm K_s$} &    7.8 & $ 8.387 \pm 0.463$ & $294664.9\pm102229.7$ \\
  316.0 & {$\rm K_s$} &    7.8 & $ 8.463 \pm 0.463$ & $274691.2\pm 95300.3$ \\
  324.0 & {$\rm K_s$} &    7.8 & $ 8.540 \pm 0.463$ & $255967.0\pm 88804.0$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UT 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{No saturated values were used in modeling.}
\end{deluxetable}


\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{KAIT Observations of GRB\,080319B\label{tab:photlogkait}}
\tablecolumns{5}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 1217.0 & {\rm clear} &   20.0 & $14.116 \pm 0.008$ & $  7008.1\pm    51.4$ \\
 1308.0 & {\rm clear} &   20.0 & $14.261 \pm 0.007$ & $  6132.0\pm    39.4$ \\
 1404.0 & {\rm clear} &   20.0 & $14.424 \pm 0.011$ & $  5277.2\pm    53.2$ \\
 1495.0 & {\rm clear} &   20.0 & $14.548 \pm 0.013$ & $  4707.6\pm    56.0$ \\
 1586.0 & {\rm clear} &   20.0 & $14.651 \pm 0.011$ & $  4281.5\pm    43.2$ \\
 1651.0 & {\rm clear} &   20.0 & $14.735 \pm 0.010$ & $  3962.8\pm    36.3$ \\
 1714.0 & {\rm clear} &   20.0 & $14.798 \pm 0.010$ & $  3739.4\pm    34.3$ \\
 1773.0 & {\rm clear} &   20.0 & $14.901 \pm 0.013$ & $  3401.0\pm    40.5$ \\
 1832.0 & {\rm clear} &   20.0 & $14.947 \pm 0.011$ & $  3259.9\pm    32.9$ \\
 1942.0 & {\rm clear} &   20.0 & $15.051 \pm 0.010$ & $  2962.1\pm    27.2$ \\
 2001.0 & {\rm clear} &   20.0 & $15.069 \pm 0.011$ & $  2913.4\pm    29.4$ \\
 2128.0 & {\rm clear} &   20.0 & $15.209 \pm 0.010$ & $  2560.9\pm    23.5$ \\
 2188.0 & {\rm clear} &   20.0 & $15.259 \pm 0.011$ & $  2445.7\pm    24.7$ \\
 2308.0 & {\rm clear} &   20.0 & $15.335 \pm 0.010$ & $  2280.3\pm    20.9$ \\
 2432.0 & {\rm clear} &   20.0 & $15.400 \pm 0.012$ & $  2147.8\pm    23.6$ \\
 2557.0 & {\rm clear} &   20.0 & $15.503 \pm 0.009$ & $  1953.4\pm    16.1$ \\
 2678.0 & {\rm clear} &   20.0 & $15.601 \pm 0.013$ & $  1784.8\pm    21.2$ \\
 2798.0 & {\rm clear} &   20.0 & $15.640 \pm 0.013$ & $  1721.9\pm    20.5$ \\
 2922.0 & {\rm clear} &   20.0 & $15.716 \pm 0.014$ & $  1605.5\pm    20.6$ \\
 3047.0 & {\rm clear} &   20.0 & $15.750 \pm 0.016$ & $  1556.0\pm    22.8$ \\
 3168.0 & {\rm clear} &   20.0 & $15.806 \pm 0.014$ & $  1477.7\pm    18.9$ \\
 3289.0 & {\rm clear} &   20.0 & $15.870 \pm 0.017$ & $  1393.2\pm    21.6$ \\
 3414.0 & {\rm clear} &   20.0 & $15.900 \pm 0.014$ & $  1355.2\pm    17.4$ \\
 3534.0 & {\rm clear} &   20.0 & $15.978 \pm 0.021$ & $  1261.2\pm    24.2$ \\
 3655.0 & {\rm clear} &   20.0 & $15.999 \pm 0.014$ & $  1237.1\pm    15.8$ \\
 3780.0 & {\rm clear} &   20.0 & $16.060 \pm 0.015$ & $  1169.5\pm    16.0$ \\
 3901.0 & {\rm clear} &   20.0 & $16.080 \pm 0.020$ & $  1148.2\pm    21.0$ \\
 4026.0 & {\rm clear} &   20.0 & $16.127 \pm 0.018$ & $  1099.5\pm    18.1$ \\
 4146.0 & {\rm clear} &   20.0 & $16.198 \pm 0.016$ & $  1029.9\pm    15.1$ \\
 4267.0 & {\rm clear} &   20.0 & $16.242 \pm 0.013$ & $   989.0\pm    11.8$ \\
 4331.0 & {\rm clear} &   20.0 & $16.262 \pm 0.017$ & $   971.0\pm    15.1$ \\
 4390.0 & {\rm clear} &   20.0 & $16.254 \pm 0.014$ & $   978.1\pm    12.5$ \\
 4449.0 & {\rm clear} &   20.0 & $16.278 \pm 0.017$ & $   956.8\pm    14.9$ \\
 4508.0 & {\rm clear} &   20.0 & $16.285 \pm 0.016$ & $   950.6\pm    13.9$ \\
 4567.0 & {\rm clear} &   20.0 & $16.334 \pm 0.014$ & $   908.7\pm    11.6$ \\
 5015.0 & {\rm clear} &   20.0 & $16.422 \pm 0.019$ & $   837.9\pm    14.5$ \\
 5114.0 & {\rm clear} &   20.0 & $16.471 \pm 0.011$ & $   800.9\pm     8.1$ \\
 5316.0 & {\rm clear} &   20.0 & $16.508 \pm 0.016$ & $   774.1\pm    11.3$ \\
 5420.0 & {\rm clear} &   20.0 & $16.541 \pm 0.017$ & $   750.9\pm    11.7$ \\
 5619.0 & {\rm clear} &   20.0 & $16.592 \pm 0.021$ & $   716.5\pm    13.7$ \\
 5823.0 & {\rm clear} &   20.0 & $16.633 \pm 0.012$ & $   689.9\pm     7.6$ \\
 6023.0 & {\rm clear} &   20.0 & $16.667 \pm 0.020$ & $   668.7\pm    12.2$ \\
 6227.0 & {\rm clear} &   20.0 & $16.739 \pm 0.017$ & $   625.7\pm     9.7$ \\
 6426.0 & {\rm clear} &   20.0 & $16.783 \pm 0.021$ & $   600.9\pm    11.5$ \\
 6631.0 & {\rm clear} &   20.0 & $16.773 \pm 0.025$ & $   606.5\pm    13.8$ \\
 6830.0 & {\rm clear} &   20.0 & $16.850 \pm 0.017$ & $   564.9\pm     8.8$ \\
 7034.0 & {\rm clear} &   20.0 & $16.892 \pm 0.022$ & $   543.5\pm    10.9$ \\
 8820.0 & {\rm clear} &  300.0 & $17.153 \pm 0.012$ & $   427.4\pm     4.7$ \\
10028.0 & {\rm clear} &  300.0 & $17.335 \pm 0.015$ & $   361.4\pm     5.0$ \\
11271.0 & {\rm clear} &  300.0 & $17.528 \pm 0.014$ & $   302.6\pm     3.9$ \\
12477.0 & {\rm clear} &  300.0 & $17.625 \pm 0.014$ & $   276.7\pm     3.5$ \\
15537.0 & {\rm clear} &  300.0 & $17.919 \pm 0.022$ & $   211.1\pm     4.2$ \\
16744.0 & {\rm clear} &  300.0 & $18.021 \pm 0.022$ & $   192.1\pm     3.9$ \\
 2098.0 & {\rm B}     &   20.0 & $15.623 \pm 0.045$ & $  2327.0\pm    94.5$ \\
 2249.0 & {\rm B}     &   20.0 & $15.750 \pm 0.041$ & $  2070.1\pm    76.7$ \\
 2373.0 & {\rm B}     &   20.0 & $15.814 \pm 0.042$ & $  1951.6\pm    74.1$ \\
 2546.5 & {\rm B}     &   40.0 & $15.911 \pm 0.037$ & $  1784.8\pm    59.8$ \\
 2791.0 & {\rm B}     &   40.0 & $16.094 \pm 0.035$ & $  1508.0\pm    47.8$ \\
 3097.3 & {\rm B}     &   60.0 & $16.305 \pm 0.031$ & $  1241.6\pm    34.9$ \\
 3465.0 & {\rm B}     &   60.0 & $16.378 \pm 0.040$ & $  1160.9\pm    42.0$ \\
 3771.5 & {\rm B}     &   40.0 & $16.574 \pm 0.043$ & $   969.2\pm    37.6$ \\
 4075.7 & {\rm B}     &   60.0 & $16.602 \pm 0.045$ & $   944.5\pm    38.3$ \\
 5493.7 & {\rm B}     &  120.0 & $17.036 \pm 0.035$ & $   633.3\pm    20.1$ \\
 6117.3 & {\rm B}     &  120.0 & $17.173 \pm 0.036$ & $   558.2\pm    18.2$ \\
 6720.7 & {\rm B}     &  120.0 & $17.412 \pm 0.068$ & $   447.9\pm    27.2$ \\
 7789.0 & {\rm B}     &  300.0 & $17.518 \pm 0.023$ & $   406.3\pm     8.5$ \\
 8984.0 & {\rm B}     &  300.0 & $17.737 \pm 0.030$ & $   332.0\pm     9.0$ \\
10236.0 & {\rm B}     &  300.0 & $17.833 \pm 0.028$ & $   303.9\pm     7.7$ \\
11435.0 & {\rm B}     &  300.0 & $18.065 \pm 0.044$ & $   245.5\pm     9.7$ \\
14508.0 & {\rm B}     &  300.0 & $18.440 \pm 0.052$ & $   173.8\pm     8.1$ \\
15707.0 & {\rm B}     &  300.0 & $18.490 \pm 0.058$ & $   166.0\pm     8.6$ \\
 1157.0 & {\rm V}     &   20.0 & $14.345 \pm 0.022$ & $  6745.3\pm   135.3$ \\
 1248.0 & {\rm V}     &   20.0 & $14.442 \pm 0.022$ & $  6168.8\pm   123.7$ \\
 1339.0 & {\rm V}     &   20.0 & $14.651 \pm 0.022$ & $  5088.6\pm   102.1$ \\
 1435.0 & {\rm V}     &   20.0 & $14.815 \pm 0.025$ & $  4375.2\pm    99.6$ \\
 1526.0 & {\rm V}     &   20.0 & $14.939 \pm 0.026$ & $  3903.0\pm    92.4$ \\
 2067.0 & {\rm V}     &   20.0 & $15.492 \pm 0.043$ & $  2345.3\pm    91.1$ \\
 2218.0 & {\rm V}     &   20.0 & $15.631 \pm 0.047$ & $  2063.5\pm    87.4$ \\
 2453.3 & {\rm V}     &   60.0 & $15.800 \pm 0.029$ & $  1766.0\pm    46.5$ \\
 2820.0 & {\rm V}     &   60.0 & $15.921 \pm 0.036$ & $  1579.8\pm    51.5$ \\
 3188.7 & {\rm V}     &   60.0 & $16.130 \pm 0.037$ & $  1303.2\pm    43.7$ \\
 3556.3 & {\rm V}     &   60.0 & $16.336 \pm 0.043$ & $  1078.0\pm    41.9$ \\
 3984.3 & {\rm V}     &   80.0 & $16.421 \pm 0.037$ & $   996.8\pm    33.4$ \\
 5332.5 & {\rm V}     &   80.0 & $16.827 \pm 0.042$ & $   685.8\pm    26.0$ \\
 5782.0 & {\rm V}     &   80.0 & $16.954 \pm 0.055$ & $   610.1\pm    30.1$ \\
 6165.5 & {\rm V}     &   80.0 & $16.989 \pm 0.047$ & $   590.7\pm    25.0$ \\
 6569.0 & {\rm V}     &   80.0 & $17.111 \pm 0.060$ & $   528.0\pm    28.4$ \\
 6973.0 & {\rm V}     &   80.0 & $17.144 \pm 0.068$ & $   512.2\pm    31.1$ \\
 8134.0 & {\rm V}     &  300.0 & $17.453 \pm 0.057$ & $   385.3\pm    19.7$ \\
 9335.0 & {\rm V}     &  300.0 & $17.629 \pm 0.069$ & $   327.6\pm    20.2$ \\
10580.0 & {\rm V}     &  300.0 & $17.776 \pm 0.019$ & $   286.2\pm     5.0$ \\
11785.0 & {\rm V}     &  300.0 & $17.958 \pm 0.031$ & $   242.0\pm     6.8$ \\
14852.0 & {\rm V}     &  300.0 & $18.223 \pm 0.029$ & $   189.6\pm     5.0$ \\
16051.0 & {\rm V}     &  300.0 & $18.370 \pm 0.038$ & $   165.6\pm     5.7$ \\
 1188.0 & {\rm I}     &   20.0 & $13.777 \pm 0.013$ & $  7502.4\pm    89.3$ \\
 1279.0 & {\rm I}     &   20.0 & $13.879 \pm 0.012$ & $  6829.7\pm    75.1$ \\
 1370.0 & {\rm I}     &   20.0 & $14.016 \pm 0.015$ & $  6020.0\pm    82.6$ \\
 1465.0 & {\rm I}     &   20.0 & $14.176 \pm 0.020$ & $  5195.2\pm    94.8$ \\
 1557.0 & {\rm I}     &   20.0 & $14.328 \pm 0.018$ & $  4516.5\pm    74.3$ \\
 1621.0 & {\rm I}     &   20.0 & $14.381 \pm 0.021$ & $  4301.3\pm    82.4$ \\
 1680.0 & {\rm I}     &   20.0 & $14.516 \pm 0.015$ & $  3798.4\pm    52.1$ \\
 1744.0 & {\rm I}     &   20.0 & $14.572 \pm 0.028$ & $  3607.4\pm    91.8$ \\
 1803.0 & {\rm I}     &   20.0 & $14.616 \pm 0.016$ & $  3464.2\pm    50.7$ \\
 1862.0 & {\rm I}     &   20.0 & $14.686 \pm 0.021$ & $  3247.9\pm    62.2$ \\
 1912.0 & {\rm I}     &   20.0 & $14.778 \pm 0.025$ & $  2984.0\pm    67.9$ \\
 1972.0 & {\rm I}     &   20.0 & $14.807 \pm 0.025$ & $  2905.4\pm    66.1$ \\
 2031.0 & {\rm I}     &   20.0 & $14.836 \pm 0.026$ & $  2828.8\pm    66.9$ \\
 2158.0 & {\rm I}     &   20.0 & $14.958 \pm 0.021$ & $  2528.1\pm    48.4$ \\
 2331.0 & {\rm I}     &   40.0 & $15.060 \pm 0.022$ & $  2301.4\pm    46.2$ \\
 2575.5 & {\rm I}     &   40.0 & $15.174 \pm 0.023$ & $  2072.0\pm    43.4$ \\
 2821.0 & {\rm I}     &   40.0 & $15.334 \pm 0.020$ & $  1788.1\pm    32.6$ \\
 3065.5 & {\rm I}     &   40.0 & $15.439 \pm 0.022$ & $  1623.3\pm    32.6$ \\
 3311.5 & {\rm I}     &   40.0 & $15.565 \pm 0.035$ & $  1445.4\pm    45.9$ \\
 3555.5 & {\rm I}     &   40.0 & $15.700 \pm 0.031$ & $  1276.4\pm    35.9$ \\
 3800.5 & {\rm I}     &   40.0 & $15.700 \pm 0.043$ & $  1276.4\pm    49.6$ \\
 4046.5 & {\rm I}     &   40.0 & $15.788 \pm 0.031$ & $  1177.1\pm    33.1$ \\
 4259.5 & {\rm I}     &   40.0 & $15.902 \pm 0.042$ & $  1059.7\pm    40.2$ \\
 4379.5 & {\rm I}     &   40.0 & $15.892 \pm 0.043$ & $  1069.5\pm    41.5$ \\
 4527.3 & {\rm I}     &   60.0 & $15.986 \pm 0.024$ & $   980.8\pm    21.4$ \\
 5002.5 & {\rm I}     &   80.0 & $16.170 \pm 0.028$ & $   827.9\pm    21.1$ \\
 5255.0 & {\rm I}     &   80.0 & $16.221 \pm 0.025$ & $   789.9\pm    18.0$ \\
 5662.0 & {\rm I}     &   80.0 & $16.296 \pm 0.024$ & $   737.2\pm    16.1$ \\
 6065.0 & {\rm I}     &   80.0 & $16.385 \pm 0.036$ & $   679.2\pm    22.2$ \\
 6469.0 & {\rm I}     &   80.0 & $16.507 \pm 0.033$ & $   607.0\pm    18.2$ \\
 6873.0 & {\rm I}     &   80.0 & $16.495 \pm 0.030$ & $   613.8\pm    16.7$ \\
 8479.0 & {\rm I}     &  300.0 & $16.841 \pm 0.017$ & $   446.3\pm     6.9$ \\
 9680.0 & {\rm I}     &  300.0 & $17.017 \pm 0.030$ & $   379.5\pm    10.3$ \\
10924.0 & {\rm I}     &  300.0 & $17.204 \pm 0.019$ & $   319.4\pm     5.5$ \\
12129.0 & {\rm I}     &  300.0 & $17.342 \pm 0.023$ & $   281.3\pm     5.9$ \\
15195.0 & {\rm I}     &  300.0 & $17.648 \pm 0.022$ & $   212.2\pm     4.3$ \\
16402.0 & {\rm I}     &  300.0 & $17.750 \pm 0.099$ & $   193.2\pm    16.8$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\end{deluxetable}

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{Nickel Observations of GRB\,080319B\label{tab:photlognickel}}
\tablecolumns{5}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 7154.7 & {\rm B}     &  360.0 & $17.365 \pm 0.005$ & $   467.7\pm     2.1$ \\
 8579.2 & {\rm B}     &  360.0 & $17.646 \pm 0.006$ & $   361.1\pm     2.0$ \\
10013.4 & {\rm B}     &  360.0 & $17.866 \pm 0.008$ & $   294.8\pm     2.2$ \\
11512.3 & {\rm B}     &  360.0 & $18.090 \pm 0.008$ & $   239.9\pm     1.8$ \\
13015.9 & {\rm B}     &  360.0 & $18.248 \pm 0.011$ & $   207.4\pm     2.1$ \\
14473.6 & {\rm B}     &  360.0 & $18.389 \pm 0.011$ & $   182.1\pm     1.8$ \\
16436.8 & {\rm B}     &  360.0 & $18.587 \pm 0.015$ & $   151.8\pm     2.1$ \\
17937.4 & {\rm B}     &  360.0 & $18.770 \pm 0.018$ & $   128.2\pm     2.1$ \\
19398.1 & {\rm B}     &  360.0 & $18.858 \pm 0.015$ & $   118.2\pm     1.6$ \\
20965.3 & {\rm B}     &  360.0 & $18.970 \pm 0.023$ & $   106.7\pm     2.2$ \\
 7444.0 & {\rm V}     &  300.0 & $17.251 \pm 0.005$ & $   464.1\pm     2.1$ \\
 8860.5 & {\rm V}     &  300.0 & $17.484 \pm 0.007$ & $   374.5\pm     2.4$ \\
10291.9 & {\rm V}     &  300.0 & $17.727 \pm 0.007$ & $   299.4\pm     1.9$ \\
11829.3 & {\rm V}     &  300.0 & $17.899 \pm 0.007$ & $   255.5\pm     1.6$ \\
13294.2 & {\rm V}     &  300.0 & $18.062 \pm 0.007$ & $   219.9\pm     1.4$ \\
14767.2 & {\rm V}     &  300.0 & $18.236 \pm 0.014$ & $   187.3\pm     2.4$ \\
16714.4 & {\rm V}     &  300.0 & $18.424 \pm 0.012$ & $   157.5\pm     1.7$ \\
18236.5 & {\rm V}     &  300.0 & $18.559 \pm 0.016$ & $   139.1\pm     2.0$ \\
19700.4 & {\rm V}     &  300.0 & $18.637 \pm 0.013$ & $   129.5\pm     1.5$ \\
22996.8 & {\rm V}     &  300.0 & $18.902 \pm 0.021$ & $   101.4\pm     1.9$ \\
 7782.0 & {\rm R}     &  300.0 & $16.991 \pm 0.006$ & $   496.1\pm     2.7$ \\
 9196.4 & {\rm R}     &  300.0 & $17.239 \pm 0.005$ & $   394.8\pm     1.8$ \\
10635.4 & {\rm R}     &  300.0 & $17.435 \pm 0.008$ & $   329.6\pm     2.4$ \\
12181.0 & {\rm R}     &  300.0 & $17.637 \pm 0.009$ & $   273.7\pm     2.3$ \\
13652.0 & {\rm R}     &  300.0 & $17.799 \pm 0.007$ & $   235.7\pm     1.5$ \\
15110.2 & {\rm R}     &  300.0 & $17.917 \pm 0.007$ & $   211.4\pm     1.4$ \\
17071.9 & {\rm R}     &  300.0 & $18.107 \pm 0.011$ & $   177.5\pm     1.8$ \\
18582.1 & {\rm R}     &  300.0 & $18.218 \pm 0.008$ & $   160.3\pm     1.2$ \\
20035.8 & {\rm R}     &  300.0 & $18.308 \pm 0.017$ & $   147.5\pm     2.3$ \\
23331.8 & {\rm R}     &  300.0 & $18.541 \pm 0.021$ & $   119.0\pm     2.3$ \\
 8122.0 & {\rm I}     &  300.0 & $16.797 \pm 0.004$ & $   464.7\pm     1.7$ \\
 9531.2 & {\rm I}     &  300.0 & $17.013 \pm 0.005$ & $   380.9\pm     1.7$ \\
10995.4 & {\rm I}     &  300.0 & $17.189 \pm 0.005$ & $   323.9\pm     1.5$ \\
12520.7 & {\rm I}     &  300.0 & $17.394 \pm 0.005$ & $   268.2\pm     1.2$ \\
14003.3 & {\rm I}     &  300.0 & $17.537 \pm 0.009$ & $   235.1\pm     1.9$ \\
15973.2 & {\rm I}     &  300.0 & $17.704 \pm 0.008$ & $   201.6\pm     1.5$ \\
17412.9 & {\rm I}     &  300.0 & $17.817 \pm 0.011$ & $   181.6\pm     1.8$ \\
18936.7 & {\rm I}     &  300.0 & $17.921 \pm 0.010$ & $   165.0\pm     1.5$ \\
20447.9 & {\rm I}     &  300.0 & $18.045 \pm 0.014$ & $   147.2\pm     1.9$ \\
23665.5 & {\rm I}     &  300.0 & $18.111 \pm 0.118$ & $   138.5\pm    14.3$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\end{deluxetable}


\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{UVOT Observations of GRB\,080319B\label{tab:photloguvot}}
\tablecolumns{5}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 6156.0 & {\rm UVW1}  &  196.6 & $16.146 \pm 0.043$ & $   343.2\pm    13.3$ \\
17398.0 & {\rm UVW1}  &  885.6 & $17.645 \pm 0.042$ & $    86.3\pm     3.3$ \\
28047.0 & {\rm UVW1}  &  427.9 & $18.316 \pm 0.086$ & $    46.5\pm     3.5$ \\
45393.0 & {\rm UVW1}  &  427.9 & $18.909 \pm 0.121$ & $    26.9\pm     2.8$ \\
75628.0 & {\rm UVW1}  &  200.6 & $19.266 \pm 0.213$ & $    19.4\pm     3.5$ \\
 5542.0 & {\rm UVW2}  &  196.6 & $16.192 \pm 0.046$ & $   239.6\pm     9.9$ \\
10709.0 & {\rm UVW2}  &  885.6 & $17.231 \pm 0.036$ & $    92.0\pm     3.0$ \\
22273.0 & {\rm UVW2}  &  266.3 & $18.394 \pm 0.116$ & $    31.5\pm     3.2$ \\
28931.0 & {\rm UVW2}  &  856.1 & $18.631 \pm 0.073$ & $    25.3\pm     1.6$ \\
46279.0 & {\rm UVW2}  &  856.1 & $19.228 \pm 0.102$ & $    14.6\pm     1.3$ \\
76050.0 & {\rm UVW2}  &  401.3 & $19.888 \pm 0.220$ & $     8.0\pm     1.5$ \\
 5951.0 & {\rm UVM2}  &  196.6 & $15.923 \pm 0.052$ & $   284.4\pm    13.3$ \\
12528.0 & {\rm UVM2}  &  334.6 & $17.144 \pm 0.071$ & $    92.4\pm     5.8$ \\
16491.0 & {\rm UVM2}  &  885.6 & $17.493 \pm 0.052$ & $    67.0\pm     3.1$ \\
30028.0 & {\rm UVM2}  &  611.2 & $18.381 \pm 0.101$ & $    29.6\pm     2.6$ \\
47376.0 & {\rm UVM2}  &  610.0 & $19.039 \pm 0.144$ & $    16.1\pm     2.0$ \\
  631.0 & {\rm U}     &   19.4 & $12.474 \pm 0.028$\tablenotemark{x} & $ 19697.0\pm   501.5$\tablenotemark{x} \\
  785.0 & {\rm U}     &   19.4 & $12.968 \pm 0.030$ & $ 12496.8\pm   340.6$ \\
 1430.0 & {\rm U}     &   19.4 & $14.108 \pm 0.042$ & $  4373.2\pm   165.9$ \\
 1591.0 & {\rm U}     &   19.5 & $14.342 \pm 0.046$ & $  3525.3\pm   146.2$ \\
 4926.0 & {\rm U}     &  196.6 & $16.015 \pm 0.029$ & $   755.1\pm    19.9$ \\
 6362.0 & {\rm U}     &  196.6 & $16.329 \pm 0.033$ & $   565.5\pm    16.9$ \\
18304.0 & {\rm U}     &  295.0 & $17.864 \pm 0.056$ & $   137.5\pm     6.9$ \\
18609.0 & {\rm U}     &  231.2 & $17.886 \pm 0.064$ & $   134.8\pm     7.7$ \\
28486.0 & {\rm U}     &  213.4 & $18.498 \pm 0.089$ & $    76.7\pm     6.0$ \\
45833.0 & {\rm U}     &  213.4 & $19.435 \pm 0.148$ & $    32.4\pm     4.1$ \\
  656.0 & {\rm B}     &    9.6 & $13.334 \pm 0.042$\tablenotemark{x} & $ 19160.2\pm   727.0$\tablenotemark{x} \\
  811.0 & {\rm B}     &    9.6 & $13.913 \pm 0.046$ & $ 11240.9\pm   466.3$ \\
 1454.0 & {\rm B}     &   19.4 & $15.012 \pm 0.046$ & $  4085.1\pm   169.5$ \\
 1616.0 & {\rm B}     &   19.5 & $15.291 \pm 0.052$ & $  3159.4\pm   147.7$ \\
 5131.0 & {\rm B}     &  196.6 & $16.962 \pm 0.033$ & $   678.0\pm    20.3$ \\
 6567.0 & {\rm B}     &  196.6 & $17.350 \pm 0.039$ & $   474.2\pm    16.7$ \\
28708.0 & {\rm B}     &  213.4 & $19.417 \pm 0.112$ & $    70.7\pm     6.9$ \\
46055.0 & {\rm B}     &  213.3 & $20.036 \pm 0.171$ & $    40.0\pm     5.8$ \\
75943.0 & {\rm B}     &  100.2 & $20.441 \pm 0.316$ & $    27.5\pm     6.9$ \\
  711.0 & {\rm V}     &   19.5 & $13.373 \pm 0.040$\tablenotemark{x} & $ 16512.0\pm   597.2$\tablenotemark{x} \\
  975.0 & {\rm V}     &  393.5 & $14.337 \pm 0.013$\tablenotemark{x} & $  6795.2\pm    80.9$\tablenotemark{x} \\
 1518.0 & {\rm V}     &   19.4 & $15.025 \pm 0.076$ & $  3605.8\pm   243.8$ \\
 1680.0 & {\rm V}     &   19.5 & $15.127 \pm 0.081$ & $  3282.5\pm   236.0$ \\
 5746.0 & {\rm V}     &  196.6 & $16.955 \pm 0.058$ & $   609.5\pm    31.7$ \\
11616.0 & {\rm V}     &  295.0 & $17.948 \pm 0.078$ & $   244.2\pm    16.9$ \\
11919.0 & {\rm V}     &  295.1 & $17.895 \pm 0.078$ & $   256.4\pm    17.8$ \\
12222.0 & {\rm V}     &  295.0 & $18.041 \pm 0.082$ & $   224.2\pm    16.3$ \\
29806.0 & {\rm V}     &  213.4 & $19.491 \pm 0.256$ & $    59.0\pm    12.4$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{Gemini Observations of GRB\,080319B\label{tab:photloggemini}}
\tablecolumns{5}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
       89309 & {\rm g} & 5 $\times$ 180 & $20.670 \pm 0.100$ & $   19.59\pm    1.72$ \\
       90356 & {\rm r} & 5 $\times$ 180 & $20.520 \pm 0.060$ & $   22.49\pm    1.21$ \\
       91307 & {\rm i} & 5 $\times$ 180 & $20.380 \pm 0.050$ & $   25.59\pm    1.15$ \\
       92470 & {\rm z} & 5 $\times$ 180 & $20.310 \pm 0.050$ & $   27.93\pm    1.26$ \\
      174960 & {\rm r} & 5 $\times$ 180 & $21.510 \pm 0.060$ & $   9.037\pm   0.486$ \\
      520390 & {\rm g} & 6 $\times$ 180 & $23.450 \pm 0.190$ & $   1.514\pm   0.243$ \\
      521589 & {\rm r} & 6 $\times$ 180 & $23.340 \pm 0.090$ & $   1.675\pm   0.133$ \\
      522792 & {\rm i} & 6 $\times$ 180 & $22.900 \pm 0.060$ & $   2.512\pm   0.135$ \\
      523990 & {\rm z} & 6 $\times$ 180 & $22.940 \pm 0.090$ & $   2.477\pm   0.197$ \\
      780120 & {\rm r} & 6 $\times$ 180 & $23.670 \pm 0.070$ & $   1.236\pm   0.077$ \\
      781560 & {\rm i} & 6 $\times$ 180 & $23.280 \pm 0.060$ & $   1.770\pm   0.095$ \\
     1209960 & {\rm g} & 6 $\times$ 180 & $24.440 \pm 0.080$ & $  0.6081\pm  0.0432$ \\
     1211220 & {\rm r} & 6 $\times$ 180 & $24.100 \pm 0.080$ & $  0.8318\pm  0.0591$ \\
     1212480 & {\rm i} & 6 $\times$ 180 & $23.810 \pm 0.070$ & $   1.086\pm   0.068$ \\
     2286720 & {\rm g} & 6 $\times$ 180 & $25.860 \pm 0.110$\tablenotemark{x} & $  0.1644\pm  0.0158$\tablenotemark{x} \\
     2287800 & {\rm r} & 6 $\times$ 180 & $25.050 \pm 0.090$\tablenotemark{x} & $  0.3467\pm  0.0276$\tablenotemark{x} \\
     2285280 & {\rm i} & 6 $\times$ 180 & $24.360 \pm 0.080$\tablenotemark{x} & $  0.6546\pm  0.0465$\tablenotemark{x} \\
     2531160 & {\rm z} & 3 $\times$ 180  & $23.940 \pm 0.130$\tablenotemark{x} & $  0.9863\pm  0.1113$\tablenotemark{x} \\
     % 4592160 & {\rm g} & 9 $\times$ 180 & $\geq 26.5$        & $         \leq  0.09$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}

\begin{deluxetable}{rccllll}
\tabletypesize{\small}
\tablecaption{GCN Observations of GRB\,080319B\label{tab:photloggcn}}
\tablecolumns{7}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} & \colhead{} & \colhead{} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy} & \colhead{} & \colhead{}}
\startdata
  -11.0 & {\rm clear} &   10.0 & $ \geq 11.48$ & $ \leq7.94\times 10^{4}$ & Pi\tablenotemark{c} & GCN 7445\tablenotemark{d}\\
    3.0 & {\rm clear} &   10.0 & $  9.83$ & $3.63\times 10^{5}$ & Pi & GCN 7445\\
   17.0 & {\rm clear} &   10.0 & $  5.76$ & $1.54\times 10^{7}$ & Pi & GCN 7445\\
   32.0 & {\rm clear} &   10.0 & $  6.00$ & $1.24\times 10^{7}$ & Pi & GCN 7445\\
   79.0 & {\rm clear} &   10.0 & $  8.26$ & $1.54\times 10^{6}$ & Pi & GCN 7445\\
   93.0 & {\rm clear} &   10.0 & $  8.77$ & $9.64\times 10^{5}$ & Pi & GCN 7445\\
  108.0 & {\rm clear} &   10.0 & $  9.10$ & $7.11\times 10^{5}$ & Pi & GCN 7445\\
  122.0 & {\rm clear} &   10.0 & $ 10.27$ & $2.42\times 10^{5}$ & Pi & GCN 7445\\
  163.0 & {\rm clear} &   10.0 & $ 10.50$ & $1.96\times 10^{5}$ & Pi & GCN 7445\\
  177.0 & {\rm clear} &   10.0 & $ 11.10$ & $1.13\times 10^{5}$ & Pi & GCN 7445\\
  252.0 & {\rm clear} &   10.0 & $ 11.21$ & $1.02\times 10^{5}$ & Pi & GCN 7445\\
  296.0 & {\rm clear} &   10.0 & $ 11.79$ & $5.97\times 10^{4}$ & Pi & GCN 7445\\
  310.0 & {\rm clear} &   10.0 & $ 11.95$ & $5.15\times 10^{4}$ & Pi & GCN 7445\\
   37.2 & {\rm clear} &   10.0 & $  5.60$ & $1.79\times 10^{7}$ & RAPTOR & GCN 7464\tablenotemark{e} \\
   24.6 & {\rm clear} &    5.0 & $  5.35$ & $2.25\times 10^{7}$ & ROTSE & GCN 7470\tablenotemark{f}\\
  111.7 & {\rm clear} &   20.0 & $  8.49$ & $1.25\times 10^{6}$ & ROTSE & GCN 7470\\
    8.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 8.198 \pm 0.579$ & $1.94\times 10^{6}\pm8.02\times 10^{5}$ & TORTORA & GCN 7558\tablenotemark{g} \\
   10.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.967 \pm 0.188$ & $6.03\times 10^{6}\pm9.58\times 10^{5}$ & TORTORA & GCN 7558\\
   11.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.650 \pm 0.141$ & $8.07\times 10^{6}\pm9.83\times 10^{5}$ & TORTORA & GCN 7558\\
   12.8 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.014 \pm 0.076$ & $1.45\times 10^{7}\pm9.80\times 10^{5}$ & TORTORA & GCN 7558\\
   14.0 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.801 \pm 0.064$ & $1.76\times 10^{7}\pm1.01\times 10^{6}$ & TORTORA & GCN 7558\\
   14.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.667 \pm 0.054$ & $2.00\times 10^{7}\pm9.69\times 10^{5}$ & TORTORA & GCN 7558\\
   15.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.493 \pm 0.049$ & $2.34\times 10^{7}\pm1.03\times 10^{6}$ & TORTORA & GCN 7558\\
   15.7 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.508 \pm 0.050$ & $2.31\times 10^{7}\pm1.04\times 10^{6}$ & TORTORA & GCN 7558\\
   16.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.473 \pm 0.050$ & $2.39\times 10^{7}\pm1.07\times 10^{6}$ & TORTORA & GCN 7558\\
   17.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.459 \pm 0.049$ & $2.42\times 10^{7}\pm1.07\times 10^{6}$ & TORTORA & GCN 7558\\
   17.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.369 \pm 0.050$ & $2.63\times 10^{7}\pm1.18\times 10^{6}$ & TORTORA & GCN 7558\\
   18.3 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.325 \pm 0.047$ & $2.74\times 10^{7}\pm1.16\times 10^{6}$ & TORTORA & GCN 7558\\
   19.2 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.444 \pm 0.045$ & $2.45\times 10^{7}\pm9.95\times 10^{5}$ & TORTORA & GCN 7558\\
   19.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.414 \pm 0.048$ & $2.52\times 10^{7}\pm1.09\times 10^{6}$ & TORTORA & GCN 7558\\
   20.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.414 \pm 0.047$ & $2.52\times 10^{7}\pm1.07\times 10^{6}$ & TORTORA & GCN 7558\\
   21.0 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.459 \pm 0.048$ & $2.42\times 10^{7}\pm1.05\times 10^{6}$ & TORTORA & GCN 7558\\
   21.8 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.399 \pm 0.053$ & $2.56\times 10^{7}\pm1.22\times 10^{6}$ & TORTORA & GCN 7558\\
   22.2 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.503 \pm 0.051$ & $2.32\times 10^{7}\pm1.07\times 10^{6}$ & TORTORA & GCN 7558\\
   23.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.667 \pm 0.054$ & $2.00\times 10^{7}\pm9.69\times 10^{5}$ & TORTORA & GCN 7558\\
   31.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.831 \pm 0.036$ & $1.72\times 10^{7}\pm5.60\times 10^{5}$ & TORTORA & GCN 7558\\
   32.8 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.955 \pm 0.039$ & $1.53\times 10^{7}\pm5.40\times 10^{5}$ & TORTORA & GCN 7558\\
   34.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.727 \pm 0.033$ & $1.89\times 10^{7}\pm5.65\times 10^{5}$ & TORTORA & GCN 7558\\
   35.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.493 \pm 0.025$ & $2.34\times 10^{7}\pm5.33\times 10^{5}$ & TORTORA & GCN 7558\\
   36.7 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.533 \pm 0.026$ & $2.26\times 10^{7}\pm5.34\times 10^{5}$ & TORTORA & GCN 7558\\
   38.0 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.598 \pm 0.028$ & $2.13\times 10^{7}\pm5.42\times 10^{5}$ & TORTORA & GCN 7558\\
   39.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.776 \pm 0.031$ & $1.81\times 10^{7}\pm5.08\times 10^{5}$ & TORTORA & GCN 7558\\
   40.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.702 \pm 0.030$ & $1.93\times 10^{7}\pm5.27\times 10^{5}$ & TORTORA & GCN 7558\\
   41.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.607 \pm 0.027$ & $2.11\times 10^{7}\pm5.18\times 10^{5}$ & TORTORA & GCN 7558\\
   43.3 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.359 \pm 0.030$ & $2.65\times 10^{7}\pm7.22\times 10^{5}$ & TORTORA & GCN 7558\\
   44.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.488 \pm 0.025$ & $2.35\times 10^{7}\pm5.36\times 10^{5}$ & TORTORA & GCN 7558\\
   45.8 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.607 \pm 0.028$ & $2.11\times 10^{7}\pm5.37\times 10^{5}$ & TORTORA & GCN 7558\\
   47.2 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.637 \pm 0.028$ & $2.05\times 10^{7}\pm5.22\times 10^{5}$ & TORTORA & GCN 7558\\
   48.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.712 \pm 0.031$ & $1.92\times 10^{7}\pm5.39\times 10^{5}$ & TORTORA & GCN 7558\\
   49.7 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.905 \pm 0.034$ & $1.60\times 10^{7}\pm4.94\times 10^{5}$ & TORTORA & GCN 7558\\
   51.0 & {\rm clear}\tablenotemark{v}     &      -- & $ 5.980 \pm 0.039$ & $1.50\times 10^{7}\pm5.28\times 10^{5}$ & TORTORA & GCN 7558\\
   52.3 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.193 \pm 0.049$ & $1.23\times 10^{7}\pm5.43\times 10^{5}$ & TORTORA & GCN 7558\\
   53.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.188 \pm 0.042$ & $1.24\times 10^{7}\pm4.69\times 10^{5}$ & TORTORA & GCN 7558\\
   54.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.352 \pm 0.053$ & $1.06\times 10^{7}\pm5.06\times 10^{5}$ & TORTORA & GCN 7558\\
   56.2 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.431 \pm 0.059$ & $9.88\times 10^{6}\pm5.22\times 10^{5}$ & TORTORA & GCN 7558\\
   57.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.650 \pm 0.069$ & $8.07\times 10^{6}\pm4.97\times 10^{5}$ & TORTORA & GCN 7558\\
   58.8 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.769 \pm 0.078$ & $7.23\times 10^{6}\pm5.01\times 10^{5}$ & TORTORA & GCN 7558\\
   60.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.888 \pm 0.085$ & $6.48\times 10^{6}\pm4.88\times 10^{5}$ & TORTORA & GCN 7558\\
   61.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 7.101 \pm 0.108$ & $5.33\times 10^{6}\pm5.05\times 10^{5}$ & TORTORA & GCN 7558\\
   62.7 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.992 \pm 0.099$ & $5.89\times 10^{6}\pm5.13\times 10^{5}$ & TORTORA & GCN 7558\\
   66.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 7.334 \pm 0.110$ & $4.30\times 10^{6}\pm4.14\times 10^{5}$ & TORTORA & GCN 7558\\
   71.6 & {\rm clear}\tablenotemark{v}     &      -- & $ 7.632 \pm 0.132$ & $3.27\times 10^{6}\pm3.74\times 10^{5}$ & TORTORA & GCN 7558\\
   76.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 8.034 \pm 0.203$ & $2.26\times 10^{6}\pm3.85\times 10^{5}$ & TORTORA & GCN 7558\\
   82.0 & {\rm clear}\tablenotemark{v}     &      -- & $ 8.600 \pm 0.330$ & $1.34\times 10^{6}\pm3.51\times 10^{5}$ & TORTORA & GCN 7558\\
   87.2 & {\rm clear}\tablenotemark{v}     &      -- & $ 8.580 \pm 0.330$ & $1.36\times 10^{6}\pm3.58\times 10^{5}$ & TORTORA & GCN 7558\\
   92.4 & {\rm clear}\tablenotemark{v}     &      -- & $ 9.002 \pm 0.498$ & $9.25\times 10^{5}\pm3.40\times 10^{5}$ & TORTORA & GCN 7558\\
   97.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 9.925 \pm 1.161$ & $3.95\times 10^{5}\pm2.60\times 10^{5}$ & TORTORA & GCN 7558\\
60300.0 & {\rm R}     &      -- & $ 19.80$           & $3.73\times 10^{1}$                     & Canarias  & GCN 7476\tablenotemark{h} \\
55830.0 & {\rm clear} & 1500.0 &  $19.080 \pm 0.020$ & $7.24\times 10^{1}\pm1.32\times 10^{0}$ & AAVSO & GCN 7484\tablenotemark{i} \\
70500.0 & {\rm clear} & 2040.0 &  $19.000 \pm 0.100$ & $7.80\times 10^{1}\pm6.86\times 10^{0}$ & AAVSO & GCN 7484 \\
74831.0 & {\rm R}     &      -- & $20.000 \pm 0.300$ & $3.10\times 10^{1}\pm7.50\times 10^{0}$ & Brno  & GCN 7504\tablenotemark{j} \\
43934.4 & {\rm R}     &      -- & $ 19.10$           & $7.11\times 10^{1}$                     & Kharkiv & GCN 7519\tablenotemark{k}  \\
46270.8 & {\rm R}     &      -- & $ 19.90$           & $3.40\times 10^{1}$                     & Kharkiv & GCN 7519   \\
71208.0 & {\rm R}     &      -- & $ 20.10$           & $2.83\times 10^{1}$                     & Kharkiv & GCN 7519   \\
1656000 & {\rm R}\tablenotemark{n}& -- & $ 24.35$           & $5.65\times 10^{-1}$                     & HST & GCN 7569\tablenotemark{l}\\
1656000 & {\rm I}\tablenotemark{o}& -- & $ 23.76$           & $7.62\times 10^{-1}$                     & HST & GCN 7569\\
4590000 & {\rm R}\tablenotemark{n}& -- & $26.280 \pm 0.100$ & $9.55\times 10^{-2}\pm8.40\times 10^{-3}$ & HST & GCN 7710\tablenotemark{m} \\
4590000 & {\rm I}\tablenotemark{o}& -- & $25.460 \pm 0.100$ & $1.59\times 10^{-1}\pm1.40\times 10^{-2}$ & HST & GCN 7710\\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the {\textit{Swift}}\, trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{c}{``Pi$-$of$-$the$-$Sky'' Collaboration.}
\tablenotetext{d}{\cite{Cwiok08_GCN7445}}
\tablenotetext{e}{\cite{Wozniak08_GCN7464}}
\tablenotetext{f}{\cite{Swan08_GCN7470}}
\tablenotetext{g}{\cite{Karpov08_GCN7558}}
\tablenotetext{h}{\cite{Jelinek08_GCN7476}}
\tablenotetext{i}{\cite{Hentunen08_GCN7484}}
\tablenotetext{j}{\cite{Novak08_GCN7504}}
\tablenotetext{k}{\cite{Krugly08_GCN7519}}
\tablenotetext{l}{\cite{Tanvir08_GCN7569}}
\tablenotetext{m}{\cite{Levan08_GCN7710}}
\tablenotetext{n}{Converted from F606W.}
\tablenotetext{o}{Converted from F804W.}
\tablenotetext{v}{Calibrated to $V$-band and plotted as $V$ in our figures.}
\tablenotetext{x}{No GCN observations were used in modeling.}
\end{deluxetable}




==> phot_short.tex <==

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Observations of GRB\,080319B\label{tab:photlogptel}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
  344.0 & {\rm J}     &    7.8 & $10.389 \pm 0.048$ & $111255.0\pm  4815.5$ \\
  352.3 & {\rm J}     &    7.8 & $10.483 \pm 0.048$ & $102084.5\pm  4419.0$ \\
  360.2 & {\rm J}     &    7.8 & $10.563 \pm 0.048$ & $ 94763.2\pm  4102.4$ \\
  380.1 & {\rm J}     &    7.8 & $10.652 \pm 0.048$ & $ 87313.1\pm  3779.8$ \\
  388.4 & {\rm J}     &    7.8 & $10.722 \pm 0.048$ & $ 81846.4\pm  3544.3$ \\
  396.3 & {\rm J}     &    7.8 & $10.781 \pm 0.048$ & $ 77538.9\pm  3357.8$ \\
  416.3 & {\rm J}     &    7.8 & $10.877 \pm 0.048$ & $ 70983.9\pm  3074.6$ \\
  424.5 & {\rm J}     &    7.8 & $10.896 \pm 0.048$ & $ 69752.5\pm  3021.6$ \\
  432.4 & {\rm J}     &    7.8 & $10.952 \pm 0.048$ & $ 66227.7\pm  2868.9$ \\
  344.0 & {\rm H}     &    7.8 & $ 9.639 \pm 0.042$ & $142696.2\pm  5421.2$ \\
  352.3 & {\rm H}     &    7.8 & $ 9.721 \pm 0.042$ & $132364.7\pm  5029.4$ \\
  360.2 & {\rm H}     &    7.8 & $ 9.753 \pm 0.042$ & $128513.3\pm  4883.6$ \\
  380.1 & {\rm H}     &    7.8 & $ 9.946 \pm 0.042$ & $107582.1\pm  4088.8$ \\
  388.4 & {\rm H}     &    7.8 & $ 9.985 \pm 0.042$ & $103750.1\pm  3944.2$ \\
  396.3 & {\rm H}     &    7.8 & $10.115 \pm 0.042$ & $ 92078.9\pm  3501.5$ \\
  416.3 & {\rm H}     &    7.8 & $10.127 \pm 0.042$ & $ 91066.8\pm  3464.2$ \\
  424.5 & {\rm H}     &    7.8 & $10.177 \pm 0.042$ & $ 86920.1\pm  3306.4$ \\
  432.4 & {\rm H}     &    7.8 & $10.245 \pm 0.042$ & $ 81665.8\pm  3107.6$ \\
  344.0 & {$\rm K_s$} &    7.8 & $ 9.067 \pm 0.058$\tablenotemark{x} & $157495.6\pm  8197.4$\tablenotemark{x} \\
  352.3 & {$\rm K_s$} &    7.8 & $ 9.308 \pm 0.058$\tablenotemark{x} & $126102.6\pm  6564.2$\tablenotemark{x} \\
  360.2 & {$\rm K_s$} &    7.8 & $ 9.207 \pm 0.058$\tablenotemark{x} & $138421.8\pm  7205.9$\tablenotemark{x} \\
  380.1 & {$\rm K_s$} &    7.8 & $ 9.312 \pm 0.058$ & $125650.6\pm  6541.1$ \\
  388.4 & {$\rm K_s$} &    7.8 & $ 9.310 \pm 0.058$ & $125949.5\pm  6557.6$ \\
  396.3 & {$\rm K_s$} &    7.8 & $ 9.419 \pm 0.058$ & $113840.4\pm  5927.9$ \\
  416.3 & {$\rm K_s$} &    7.8 & $ 9.508 \pm 0.058$ & $104946.6\pm  5465.3$ \\
  424.5 & {$\rm K_s$} &    7.8 & $ 9.546 \pm 0.058$ & $101331.5\pm  5277.5$ \\
  432.4 & {$\rm K_s$} &    7.8 & $ 9.638 \pm 0.058$ & $ 93031.2\pm  4845.6$ \\
\enddata 
\tablecomments{Because of the very large number of exposures acquired, only a few representative points are given.  The full table of photometry containing all 406 points is available online.  Includes only non-saturated exposures; photometry from the saturated epochs is given in Tables \ref{tab:shortr} and \ref{tab:annulus}.}
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
%%\tablenotetext{s}{Saturated epoch; magnitude estimated via annulus photometry.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}


\begin{deluxetable}{lccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Short-Read Observations of GRB\,080319B During Saturated Regime \label{tab:shortr}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
   59.3 & {\rm J}     &  0.051 & $ 5.206 \pm 0.055$ & $1.32\times 10^{7}\pm6.52\times 10^{5}$ \\
   67.3 & {\rm J}     &  0.051 & $ 5.627 \pm 0.055$ & $8.94\times 10^{6}\pm4.43\times 10^{5}$ \\
   87.3 & {\rm J}     &  0.051 & $ 6.470 \pm 0.055$ & $4.11\times 10^{6}\pm2.04\times 10^{5}$ \\
   95.5 & {\rm J}     &  0.051 & $ 6.847 \pm 0.056$ & $2.91\times 10^{6}\pm1.45\times 10^{5}$ \\
  103.5 & {\rm J}     &  0.051 & $ 6.954 \pm 0.056$ & $2.63\times 10^{6}\pm1.32\times 10^{5}$ \\
   59.3 & {\rm H}     &  0.051 & $ 4.520 \pm 0.052$ & $1.59\times 10^{7}\pm7.47\times 10^{5}$ \\
   67.3 & {\rm H}     &  0.051 & $ 4.853 \pm 0.052$ & $1.17\times 10^{7}\pm5.50\times 10^{5}$ \\
   87.3 & {\rm H}     &  0.051 & $ 5.713 \pm 0.052$ & $5.30\times 10^{6}\pm2.50\times 10^{5}$ \\
   95.5 & {\rm H}     &  0.051 & $ 6.101 \pm 0.052$ & $3.71\times 10^{6}\pm1.75\times 10^{5}$ \\
  103.5 & {\rm H}     &  0.051 & $ 6.225 \pm 0.052$ & $3.31\times 10^{6}\pm1.56\times 10^{5}$ \\
   67.3 & {$\rm K_s$} &  0.051 & $ 4.362 \pm 0.048$ & $1.20\times 10^{7}\pm5.20\times 10^{5}$ \\
   87.3 & {$\rm K_s$} &  0.051 & $ 5.192 \pm 0.048$ & $5.59\times 10^{6}\pm2.43\times 10^{5}$ \\
   95.5 & {$\rm K_s$} &  0.051 & $ 5.308 \pm 0.048$ & $5.02\times 10^{6}\pm2.18\times 10^{5}$ \\
  103.5 & {$\rm K_s$} &  0.051 & $ 5.675 \pm 0.048$ & $3.58\times 10^{6}\pm1.56\times 10^{5}$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UT 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{No saturated values were used in modeling.}
\tablecomments{Because of the large number of exposures acquired, only a few representative points are given.  The full table of photometry containing all 406 points is available online.}
\end{deluxetable}

\begin{deluxetable}{lccll}
\tabletypesize{\small}
\tablecaption{PAIRITEL Annulus Photometry of GRB\,080319B During Saturated Regime\label{tab:annulus}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
   55.0 & {\rm J}     &    7.8 & $ 4.595 \pm 0.133$ & $2.31\times 10^{7}\pm2.66\times 10^{6}$ \\
   63.2 & {\rm J}     &    7.8 & $ 5.070 \pm 0.133$ & $1.49\times 10^{7}\pm1.72\times 10^{6}$ \\
   71.2 & {\rm J}     &    7.8 & $ 5.560 \pm 0.133$ & $9.51\times 10^{6}\pm1.10\times 10^{6}$ \\
   91.2 & {\rm J}     &    7.8 & $ 6.572 \pm 0.133$ & $3.74\times 10^{6}\pm4.31\times 10^{5}$ \\
   99.4 & {\rm J}     &    7.8 & $ 6.710 \pm 0.133$ & $3.30\times 10^{6}\pm3.80\times 10^{5}$ \\
  107.4 & {\rm J}     &    7.8 & $ 7.004 \pm 0.133$ & $2.51\times 10^{6}\pm2.90\times 10^{5}$ \\
   55.0 & {\rm H}     &    7.8 & $ 4.387 \pm 0.191$ & $1.80\times 10^{7}\pm2.90\times 10^{6}$ \\
   63.2 & {\rm H}     &    7.8 & $ 4.805 \pm 0.191$ & $1.22\times 10^{7}\pm1.97\times 10^{6}$ \\
   71.2 & {\rm H}     &    7.8 & $ 5.159 \pm 0.191$ & $8.84\times 10^{6}\pm1.42\times 10^{6}$ \\
   91.2 & {\rm H}     &    7.8 & $ 5.818 \pm 0.191$ & $4.82\times 10^{6}\pm7.76\times 10^{5}$ \\
   99.4 & {\rm H}     &    7.8 & $ 6.386 \pm 0.191$ & $2.86\times 10^{6}\pm4.60\times 10^{5}$ \\
  107.4 & {\rm H}     &    7.8 & $ 6.421 \pm 0.191$ & $2.76\times 10^{6}\pm4.45\times 10^{5}$ \\
   55.0 & {$\rm K_s$} &    7.8 & $ 3.853 \pm 0.463$ & $1.92\times 10^{7}\pm6.65\times 10^{6}$ \\
   63.2 & {$\rm K_s$} &    7.8 & $ 4.200 \pm 0.463$ & $1.39\times 10^{7}\pm4.83\times 10^{6}$ \\
   71.2 & {$\rm K_s$} &    7.8 & $ 4.510 \pm 0.463$ & $1.05\times 10^{7}\pm3.63\times 10^{6}$ \\
   91.2 & {$\rm K_s$} &    7.8 & $ 5.130 \pm 0.463$ & $5.91\times 10^{6}\pm2.05\times 10^{6}$ \\
   99.4 & {$\rm K_s$} &    7.8 & $ 5.659 \pm 0.463$ & $3.63\times 10^{6}\pm1.26\times 10^{6}$ \\
  107.4 & {$\rm K_s$} &    7.8 & $ 5.812 \pm 0.463$ & $3.16\times 10^{6}\pm1.09\times 10^{6}$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UT 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{No saturated values were used in modeling.}
\tablecomments{Because of the large number of exposures acquired, only a few representative points are given.  The full table of photometry containing all 406 points is available online.}
\end{deluxetable}



\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{KAIT Observations of GRB\,080319B\label{tab:photlogkait}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 1217.0 & {\rm clear} &   20.0 & $14.116 \pm 0.008$ & $  7008.1\pm    51.4$ \\
 1308.0 & {\rm clear} &   20.0 & $14.261 \pm 0.007$ & $  6132.0\pm    39.4$ \\
 1404.0 & {\rm clear} &   20.0 & $14.424 \pm 0.011$ & $  5277.2\pm    53.2$ \\
 1495.0 & {\rm clear} &   20.0 & $14.548 \pm 0.013$ & $  4707.6\pm    56.0$ \\
 1586.0 & {\rm clear} &   20.0 & $14.651 \pm 0.011$ & $  4281.5\pm    43.2$ \\
 2098.0 & {\rm B}     &   20.0 & $15.623 \pm 0.045$ & $  2327.0\pm    94.5$ \\
 2249.0 & {\rm B}     &   20.0 & $15.750 \pm 0.041$ & $  2070.1\pm    76.7$ \\
 2373.0 & {\rm B}     &   20.0 & $15.814 \pm 0.042$ & $  1951.6\pm    74.1$ \\
 2546.5 & {\rm B}     &   40.0 & $15.911 \pm 0.037$ & $  1784.8\pm    59.8$ \\
 2791.0 & {\rm B}     &   40.0 & $16.094 \pm 0.035$ & $  1508.0\pm    47.8$ \\
 1157.0 & {\rm V}     &   20.0 & $14.345 \pm 0.022$ & $  6745.3\pm   135.3$ \\
 1248.0 & {\rm V}     &   20.0 & $14.442 \pm 0.022$ & $  6168.8\pm   123.7$ \\
 1339.0 & {\rm V}     &   20.0 & $14.651 \pm 0.022$ & $  5088.6\pm   102.1$ \\
 1435.0 & {\rm V}     &   20.0 & $14.815 \pm 0.025$ & $  4375.2\pm    99.6$ \\
 1526.0 & {\rm V}     &   20.0 & $14.939 \pm 0.026$ & $  3903.0\pm    92.4$ \\
 1188.0 & {\rm I}     &   20.0 & $13.777 \pm 0.013$ & $  7502.4\pm    89.3$ \\
 1279.0 & {\rm I}     &   20.0 & $13.879 \pm 0.012$ & $  6829.7\pm    75.1$ \\
 1370.0 & {\rm I}     &   20.0 & $14.016 \pm 0.015$ & $  6020.0\pm    82.6$ \\
 1465.0 & {\rm I}     &   20.0 & $14.176 \pm 0.020$ & $  5195.2\pm    94.8$ \\
 1557.0 & {\rm I}     &   20.0 & $14.328 \pm 0.018$ & $  4516.5\pm    74.3$ \\
\enddata 
\tablecomments{Because of the very large number of exposures acquired, only the first five exposures in each band are given.  The full table of photometry is available online.}
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\end{deluxetable}

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{Nickel Observations of GRB\,080319B\label{tab:photlognickel}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 7154.7 & {\rm B}     &  360.0 & $17.365 \pm 0.005$ & $   467.7\pm     2.1$ \\
 8579.2 & {\rm B}     &  360.0 & $17.646 \pm 0.006$ & $   361.1\pm     2.0$ \\
10013.4 & {\rm B}     &  360.0 & $17.866 \pm 0.008$ & $   294.8\pm     2.2$ \\
11512.3 & {\rm B}     &  360.0 & $18.090 \pm 0.008$ & $   239.9\pm     1.8$ \\
13015.9 & {\rm B}     &  360.0 & $18.248 \pm 0.011$ & $   207.4\pm     2.1$ \\
14473.6 & {\rm B}     &  360.0 & $18.389 \pm 0.011$ & $   182.1\pm     1.8$ \\
16436.8 & {\rm B}     &  360.0 & $18.587 \pm 0.015$ & $   151.8\pm     2.1$ \\
17937.4 & {\rm B}     &  360.0 & $18.770 \pm 0.018$ & $   128.2\pm     2.1$ \\
19398.1 & {\rm B}     &  360.0 & $18.858 \pm 0.015$ & $   118.2\pm     1.6$ \\
20965.3 & {\rm B}     &  360.0 & $18.970 \pm 0.023$ & $   106.7\pm     2.2$ \\
 7444.0 & {\rm V}     &  300.0 & $17.251 \pm 0.005$ & $   464.1\pm     2.1$ \\
 8860.5 & {\rm V}     &  300.0 & $17.484 \pm 0.007$ & $   374.5\pm     2.4$ \\
10291.9 & {\rm V}     &  300.0 & $17.727 \pm 0.007$ & $   299.4\pm     1.9$ \\
11829.3 & {\rm V}     &  300.0 & $17.899 \pm 0.007$ & $   255.5\pm     1.6$ \\
13294.2 & {\rm V}     &  300.0 & $18.062 \pm 0.007$ & $   219.9\pm     1.4$ \\
14767.2 & {\rm V}     &  300.0 & $18.236 \pm 0.014$ & $   187.3\pm     2.4$ \\
16714.4 & {\rm V}     &  300.0 & $18.424 \pm 0.012$ & $   157.5\pm     1.7$ \\
18236.5 & {\rm V}     &  300.0 & $18.559 \pm 0.016$ & $   139.1\pm     2.0$ \\
19700.4 & {\rm V}     &  300.0 & $18.637 \pm 0.013$ & $   129.5\pm     1.5$ \\
22996.8 & {\rm V}     &  300.0 & $18.902 \pm 0.021$ & $   101.4\pm     1.9$ \\
 7782.0 & {\rm R}     &  300.0 & $16.991 \pm 0.006$ & $   496.1\pm     2.7$ \\
 9196.4 & {\rm R}     &  300.0 & $17.239 \pm 0.005$ & $   394.8\pm     1.8$ \\
10635.4 & {\rm R}     &  300.0 & $17.435 \pm 0.008$ & $   329.6\pm     2.4$ \\
12181.0 & {\rm R}     &  300.0 & $17.637 \pm 0.009$ & $   273.7\pm     2.3$ \\
13652.0 & {\rm R}     &  300.0 & $17.799 \pm 0.007$ & $   235.7\pm     1.5$ \\
15110.2 & {\rm R}     &  300.0 & $17.917 \pm 0.007$ & $   211.4\pm     1.4$ \\
17071.9 & {\rm R}     &  300.0 & $18.107 \pm 0.011$ & $   177.5\pm     1.8$ \\
18582.1 & {\rm R}     &  300.0 & $18.218 \pm 0.008$ & $   160.3\pm     1.2$ \\
20035.8 & {\rm R}     &  300.0 & $18.308 \pm 0.017$ & $   147.5\pm     2.3$ \\
23331.8 & {\rm R}     &  300.0 & $18.541 \pm 0.021$ & $   119.0\pm     2.3$ \\
 8122.0 & {\rm I}     &  300.0 & $16.797 \pm 0.004$ & $   464.7\pm     1.7$ \\
 9531.2 & {\rm I}     &  300.0 & $17.013 \pm 0.005$ & $   380.9\pm     1.7$ \\
10995.4 & {\rm I}     &  300.0 & $17.189 \pm 0.005$ & $   323.9\pm     1.5$ \\
12520.7 & {\rm I}     &  300.0 & $17.394 \pm 0.005$ & $   268.2\pm     1.2$ \\
14003.3 & {\rm I}     &  300.0 & $17.537 \pm 0.009$ & $   235.1\pm     1.9$ \\
15973.2 & {\rm I}     &  300.0 & $17.704 \pm 0.008$ & $   201.6\pm     1.5$ \\
17412.9 & {\rm I}     &  300.0 & $17.817 \pm 0.011$ & $   181.6\pm     1.8$ \\
18936.7 & {\rm I}     &  300.0 & $17.921 \pm 0.010$ & $   165.0\pm     1.5$ \\
20447.9 & {\rm I}     &  300.0 & $18.045 \pm 0.014$ & $   147.2\pm     1.9$ \\
23665.5 & {\rm I}     &  300.0 & $18.111 \pm 0.118$ & $   138.5\pm    14.3$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\end{deluxetable}


\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{UVOT Observations of GRB\,080319B\label{tab:photloguvot}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
 6156.0 & {\rm UVW1}  &  196.6 & $16.146 \pm 0.043$ & $   343.2\pm    13.3$ \\
17398.0 & {\rm UVW1}  &  885.6 & $17.645 \pm 0.042$ & $    86.3\pm     3.3$ \\
28047.0 & {\rm UVW1}  &  427.9 & $18.316 \pm 0.086$ & $    46.5\pm     3.5$ \\
45393.0 & {\rm UVW1}  &  427.9 & $18.909 \pm 0.121$ & $    26.9\pm     2.8$ \\
75628.0 & {\rm UVW1}  &  200.6 & $19.266 \pm 0.213$ & $    19.4\pm     3.5$ \\
 5542.0 & {\rm UVW2}  &  196.6 & $16.192 \pm 0.046$ & $   239.6\pm     9.9$ \\
10709.0 & {\rm UVW2}  &  885.6 & $17.231 \pm 0.036$ & $    92.0\pm     3.0$ \\
22273.0 & {\rm UVW2}  &  266.3 & $18.394 \pm 0.116$ & $    31.5\pm     3.2$ \\
28931.0 & {\rm UVW2}  &  856.1 & $18.631 \pm 0.073$ & $    25.3\pm     1.6$ \\
46279.0 & {\rm UVW2}  &  856.1 & $19.228 \pm 0.102$ & $    14.6\pm     1.3$ \\
76050.0 & {\rm UVW2}  &  401.3 & $19.888 \pm 0.220$ & $     8.0\pm     1.5$ \\
 5951.0 & {\rm UVM2}  &  196.6 & $15.923 \pm 0.052$ & $   284.4\pm    13.3$ \\
12528.0 & {\rm UVM2}  &  334.6 & $17.144 \pm 0.071$ & $    92.4\pm     5.8$ \\
16491.0 & {\rm UVM2}  &  885.6 & $17.493 \pm 0.052$ & $    67.0\pm     3.1$ \\
30028.0 & {\rm UVM2}  &  611.2 & $18.381 \pm 0.101$ & $    29.6\pm     2.6$ \\
47376.0 & {\rm UVM2}  &  610.0 & $19.039 \pm 0.144$ & $    16.1\pm     2.0$ \\
  631.0 & {\rm U}     &   19.4 & $12.474 \pm 0.028$\tablenotemark{x} & $ 19697.0\pm   501.5$\tablenotemark{x} \\
  785.0 & {\rm U}     &   19.4 & $12.968 \pm 0.030$ & $ 12496.8\pm   340.6$ \\
 1430.0 & {\rm U}     &   19.4 & $14.108 \pm 0.042$ & $  4373.2\pm   165.9$ \\
 1591.0 & {\rm U}     &   19.5 & $14.342 \pm 0.046$ & $  3525.3\pm   146.2$ \\
 4926.0 & {\rm U}     &  196.6 & $16.015 \pm 0.029$ & $   755.1\pm    19.9$ \\
 6362.0 & {\rm U}     &  196.6 & $16.329 \pm 0.033$ & $   565.5\pm    16.9$ \\
18304.0 & {\rm U}     &  295.0 & $17.864 \pm 0.056$ & $   137.5\pm     6.9$ \\
18609.0 & {\rm U}     &  231.2 & $17.886 \pm 0.064$ & $   134.8\pm     7.7$ \\
28486.0 & {\rm U}     &  213.4 & $18.498 \pm 0.089$ & $    76.7\pm     6.0$ \\
45833.0 & {\rm U}     &  213.4 & $19.435 \pm 0.148$ & $    32.4\pm     4.1$ \\
  656.0 & {\rm B}     &    9.6 & $13.334 \pm 0.042$\tablenotemark{x} & $ 19160.2\pm   727.0$\tablenotemark{x} \\
  811.0 & {\rm B}     &    9.6 & $13.913 \pm 0.046$ & $ 11240.9\pm   466.3$ \\
 1454.0 & {\rm B}     &   19.4 & $15.012 \pm 0.046$ & $  4085.1\pm   169.5$ \\
 1616.0 & {\rm B}     &   19.5 & $15.291 \pm 0.052$ & $  3159.4\pm   147.7$ \\
 5131.0 & {\rm B}     &  196.6 & $16.962 \pm 0.033$ & $   678.0\pm    20.3$ \\
 6567.0 & {\rm B}     &  196.6 & $17.350 \pm 0.039$ & $   474.2\pm    16.7$ \\
28708.0 & {\rm B}     &  213.4 & $19.417 \pm 0.112$ & $    70.7\pm     6.9$ \\
46055.0 & {\rm B}     &  213.3 & $20.036 \pm 0.171$ & $    40.0\pm     5.8$ \\
75943.0 & {\rm B}     &  100.2 & $20.441 \pm 0.316$ & $    27.5\pm     6.9$ \\
  711.0 & {\rm V}     &   19.5 & $13.373 \pm 0.040$\tablenotemark{x} & $ 16512.0\pm   597.2$\tablenotemark{x} \\
  975.0 & {\rm V}     &  393.5 & $14.337 \pm 0.013$\tablenotemark{x} & $  6795.2\pm    80.9$\tablenotemark{x} \\
 1518.0 & {\rm V}     &   19.4 & $15.025 \pm 0.076$ & $  3605.8\pm   243.8$ \\
 1680.0 & {\rm V}     &   19.5 & $15.127 \pm 0.081$ & $  3282.5\pm   236.0$ \\
 5746.0 & {\rm V}     &  196.6 & $16.955 \pm 0.058$ & $   609.5\pm    31.7$ \\
11616.0 & {\rm V}     &  295.0 & $17.948 \pm 0.078$ & $   244.2\pm    16.9$ \\
11919.0 & {\rm V}     &  295.1 & $17.895 \pm 0.078$ & $   256.4\pm    17.8$ \\
12222.0 & {\rm V}     &  295.0 & $18.041 \pm 0.082$ & $   224.2\pm    16.3$ \\
29806.0 & {\rm V}     &  213.4 & $19.491 \pm 0.256$ & $    59.0\pm    12.4$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}

\begin{deluxetable}{rccll}
\tabletypesize{\small}
\tablecaption{Gemini Observations of GRB\,080319B\label{tab:photloggemini}}
\tablecolumns{6}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} &
\colhead{$\mu$Jy}}
\startdata
       89309 & {\rm g} & 5 $\times$ 180 & $20.670 \pm 0.100$ & $   19.59\pm    1.72$ \\
       90356 & {\rm r} & 5 $\times$ 180 & $20.520 \pm 0.060$ & $   22.49\pm    1.21$ \\
       91307 & {\rm i} & 5 $\times$ 180 & $20.380 \pm 0.050$ & $   25.59\pm    1.15$ \\
       92470 & {\rm z} & 5 $\times$ 180 & $20.310 \pm 0.050$ & $   27.93\pm    1.26$ \\
      174960 & {\rm r} & 5 $\times$ 180 & $21.510 \pm 0.060$ & $   9.037\pm   0.486$ \\
      520390 & {\rm g} & 6 $\times$ 180 & $23.450 \pm 0.190$ & $   1.514\pm   0.243$ \\
      521589 & {\rm r} & 6 $\times$ 180 & $23.340 \pm 0.090$ & $   1.675\pm   0.133$ \\
      522792 & {\rm i} & 6 $\times$ 180 & $22.900 \pm 0.060$ & $   2.512\pm   0.135$ \\
      523990 & {\rm z} & 6 $\times$ 180 & $22.940 \pm 0.090$ & $   2.477\pm   0.197$ \\
      780120 & {\rm r} & 6 $\times$ 180 & $23.670 \pm 0.070$ & $   1.236\pm   0.077$ \\
      781560 & {\rm i} & 6 $\times$ 180 & $23.280 \pm 0.060$ & $   1.770\pm   0.095$ \\
     1209960 & {\rm g} & 6 $\times$ 180 & $24.440 \pm 0.080$ & $  0.6081\pm  0.0432$ \\
     1211220 & {\rm r} & 6 $\times$ 180 & $24.100 \pm 0.080$ & $  0.8318\pm  0.0591$ \\
     1212480 & {\rm i} & 6 $\times$ 180 & $23.810 \pm 0.070$ & $   1.086\pm   0.068$ \\
     2286720 & {\rm g} & 6 $\times$ 180 & $25.860 \pm 0.110$\tablenotemark{x} & $  0.1644\pm  0.0158$\tablenotemark{x} \\
     2287800 & {\rm r} & 6 $\times$ 180 & $25.050 \pm 0.090$\tablenotemark{x} & $  0.3467\pm  0.0276$\tablenotemark{x} \\
     2285280 & {\rm i} & 6 $\times$ 180 & $24.360 \pm 0.080$\tablenotemark{x} & $  0.6546\pm  0.0465$\tablenotemark{x} \\
     2531160 & {\rm z} & 3 $\times$ 180 & $23.940 \pm 0.130$\tablenotemark{x} & $  0.9863\pm  0.1113$\tablenotemark{x} \\
     % 4592160 & {\rm g} & 9 $\times$ 180 & $\geq 26.5$        & $         \leq  0.09$ \\
\enddata 
\tablenotetext{a}{Exposure mid-time, measured from the \emph{Swift} trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{x}{Point not used in modeling.}
\end{deluxetable}

\begin{deluxetable}{rccllll}
\tabletypesize{\small}
\tablecaption{GCN Observations of GRB\,080319B\label{tab:photloggcn}}
\tablecolumns{7}
\tablehead{
\colhead{$t_{\rm mid}$\tablenotemark{a}} & \colhead{Filter} &
\colhead{Exp.~time} &
\colhead{Mag.\tablenotemark{b}} & \colhead{Flux\tablenotemark{b}} & \colhead{} & \colhead{} \\
\colhead{sec} & \colhead{} &
\colhead{sec} & \colhead{} & 
\colhead{$\mu$Jy} & \colhead{} & \colhead{} }
\startdata
  -11.0 & {\rm clear} &   10.0 & $ \geq 11.48$ & $ \leq7.94\times 10^{4}$ & Pi\tablenotemark{c} & GCN 7445\tablenotemark{d}\\
    3.0 & {\rm clear} &   10.0 & $  9.83$ & $3.63\times 10^{5}$ & Pi & GCN 7445\\
   17.0 & {\rm clear} &   10.0 & $  5.76$ & $1.54\times 10^{7}$ & Pi & GCN 7445\\
   32.0 & {\rm clear} &   10.0 & $  6.00$ & $1.24\times 10^{7}$ & Pi & GCN 7445\\
   79.0 & {\rm clear} &   10.0 & $  8.26$ & $1.54\times 10^{6}$ & Pi & GCN 7445\\
   93.0 & {\rm clear} &   10.0 & $  8.77$ & $9.64\times 10^{5}$ & Pi & GCN 7445\\
  108.0 & {\rm clear} &   10.0 & $  9.10$ & $7.11\times 10^{5}$ & Pi & GCN 7445\\
  122.0 & {\rm clear} &   10.0 & $ 10.27$ & $2.42\times 10^{5}$ & Pi & GCN 7445\\
  163.0 & {\rm clear} &   10.0 & $ 10.50$ & $1.96\times 10^{5}$ & Pi & GCN 7445\\
  177.0 & {\rm clear} &   10.0 & $ 11.10$ & $1.13\times 10^{5}$ & Pi & GCN 7445\\
  252.0 & {\rm clear} &   10.0 & $ 11.21$ & $1.02\times 10^{5}$ & Pi & GCN 7445\\
  296.0 & {\rm clear} &   10.0 & $ 11.79$ & $5.97\times 10^{4}$ & Pi & GCN 7445\\
  310.0 & {\rm clear} &   10.0 & $ 11.95$ & $5.15\times 10^{4}$ & Pi & GCN 7445\\
   37.2 & {\rm clear} &   10.0 & $  5.60$ & $1.79\times 10^{7}$ & RAPTOR & GCN 7464\tablenotemark{e} \\
   24.6 & {\rm clear} &    5.0 & $  5.35$ & $2.25\times 10^{7}$ & ROTSE & GCN 7470\tablenotemark{f}\\
  111.7 & {\rm clear} &   20.0 & $  8.49$ & $1.25\times 10^{6}$ & ROTSE & GCN 7470\\
    8.9 & {\rm clear}\tablenotemark{v}     &      -- & $ 8.198 \pm 0.579$ & $1.94\times 10^{6}\pm8.02\times 10^{5}$ & TORTORA & GCN 7558\tablenotemark{g} \\
   10.1 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.967 \pm 0.188$ & $6.03\times 10^{6}\pm9.58\times 10^{5}$ & TORTORA & GCN 7558\\
   11.5 & {\rm clear}\tablenotemark{v}     &      -- & $ 6.650 \pm 0.141$ & $8.07\times 10^{6}\pm9.83\times 10^{5}$ & TORTORA & GCN 7558\\
60300.0 & {\rm R}     &      -- & $ 19.80$           & $3.73\times 10^{1}$                     & Canarias  & GCN 7476\tablenotemark{h} \\
55830.0 & {\rm clear} & 1500.0 &  $19.080 \pm 0.020$ & $7.24\times 10^{1}\pm1.32\times 10^{0}$ & AAVSO & GCN 7484\tablenotemark{i} \\
70500.0 & {\rm clear} & 2040.0 &  $19.000 \pm 0.100$ & $7.80\times 10^{1}\pm6.86\times 10^{0}$ & AAVSO & GCN 7484 \\
74831.0 & {\rm R}     &      -- & $20.000 \pm 0.300$ & $3.10\times 10^{1}\pm7.50\times 10^{0}$ & Brno  & GCN 7504\tablenotemark{j} \\
43934.4 & {\rm R}     &      -- & $ 19.10$           & $7.11\times 10^{1}$                     & Kharkiv & GCN 7519\tablenotemark{k}  \\
46270.8 & {\rm R}     &      -- & $ 19.90$           & $3.40\times 10^{1}$                     & Kharkiv & GCN 7519   \\
71208.0 & {\rm R}     &      -- & $ 20.10$           & $2.83\times 10^{1}$                     & Kharkiv & GCN 7519   \\
1656000 & {\rm R}\tablenotemark{n}& -- & $ 24.35$           & $5.65\times 10^{-1}$                     & HST & GCN 7569\tablenotemark{l}\\
1656000 & {\rm I}\tablenotemark{o}& -- & $ 23.76$           & $7.62\times 10^{-1}$                     & HST & GCN 7569\\
4590000 & {\rm R}\tablenotemark{n}& -- & $26.280 \pm 0.100$ & $9.55\times 10^{-2}\pm8.40\times 10^{-3}$ & HST & GCN 7710\tablenotemark{m} \\
4590000 & {\rm I}\tablenotemark{o}& -- & $25.460 \pm 0.100$ & $1.59\times 10^{-1}\pm1.40\times 10^{-2}$ & HST & GCN 7710\\
\enddata 
\tablecomments{Most of the TORTORA measurements have been omitted to save space.  The full table of GCN photometry used in our plot is available online.}
\tablenotetext{a}{Exposure mid-time, measured from the {\textit{Swift}}\, trigger (UTC 06:12:49).}
\tablenotetext{b}{Observed value; not corrected for Galactic extinction.}
\tablenotetext{c}{``Pi$-$of$-$the$-$Sky'' Collaboration}
\tablenotetext{d}{\cite{Cwiok08_GCN7445}}
\tablenotetext{e}{\cite{Wozniak08_GCN7464}}
\tablenotetext{f}{\cite{Swan08_GCN7470}}
\tablenotetext{g}{\cite{Karpov08_GCN7558}}
\tablenotetext{h}{\cite{Jelinek08_GCN7476}}
\tablenotetext{i}{\cite{Hentunen08_GCN7484}}
\tablenotetext{j}{\cite{Novak08_GCN7504}}
\tablenotetext{k}{\cite{Krugly08_GCN7519}}
\tablenotetext{l}{\cite{Tanvir08_GCN7569}}
\tablenotetext{m}{\cite{Levan08_GCN7710}}
\tablenotetext{n}{Converted from F606W.}
\tablenotetext{o}{Converted from F804W.}
\tablenotetext{v}{Calibrated to $V$-band and plotted as $V$ in our figures.}
\tablenotetext{x}{No GCN observations were used in modeling.}
\end{deluxetable}




==> stds.tex <==

\begin{deluxetable}{llllll}
\tabletypesize{\small}
\tablecaption{Bright SDSS standard stars}
\tablecolumns{6}
\tablehead{
\colhead{RA} & \colhead{Dec} & \colhead{B} & \colhead{V} & \colhead{R} & \colhead{I}  \\
\colhead{deg} & \colhead{deg} & \colhead{mag} & \colhead{mag} & \colhead{mag} & \colhead{mag}
}
\startdata
217.915229 & 36.31513  & 15.940 $\pm$ 0.010 & 15.293 $\pm$ 0.006 &14.922 $\pm$ 0.008 & 14.551 $\pm$ 0.007 \\
217.908143 & 36.29125  & 17.716 $\pm$ 0.012 & 16.350 $\pm$ 0.006 &15.523 $\pm$ 0.008 & 14.821 $\pm$ 0.007 \\
217.943617 & 36.31667  & 17.993 $\pm$ 0.012 & 16.834 $\pm$ 0.006 &16.162 $\pm$ 0.008 & 15.590 $\pm$ 0.007 \\
\enddata 
\label{tab:lickstars}
\end{deluxetable}


\begin{deluxetable}{llllll}
\tabletypesize{\small}
\tablecaption{Faint SDSS standard stars}
\tablecolumns{6}
\tablehead{
\colhead{RA} & \colhead{Dec} & \colhead{g} & \colhead{r} & \colhead{i} & \colhead{z}  \\
\colhead{deg} & \colhead{deg} & \colhead{mag} & \colhead{mag} & \colhead{mag} & \colhead{mag}
}
\startdata
217.908143 & 36.29125 & 17.091 $\pm$ 0.005 & 15.816 $\pm$ 0.004 & 15.310 $\pm$ 0.004 & 15.067 $\pm$ 0.005 \\
217.943617 & 36.31667 & 17.425 $\pm$ 0.005 & 16.409 $\pm$ 0.004 & 16.058 $\pm$ 0.004 & 15.872 $\pm$ 0.007 \\
217.871828 & 36.29380 & 17.364 $\pm$ 0.005 & 16.903 $\pm$ 0.005 & 16.769 $\pm$ 0.005 & 16.689 $\pm$ 0.010 \\
217.894280 & 36.34851 & 18.298 $\pm$ 0.007 & 16.955 $\pm$ 0.005 & 16.370 $\pm$ 0.005 & 16.036 $\pm$ 0.007 \\
217.902832 & 36.33332 & 18.084 $\pm$ 0.006 & 17.741 $\pm$ 0.006 & 17.626 $\pm$ 0.007 & 17.565 $\pm$ 0.017 \\
217.981086 & 36.29605 & 18.223 $\pm$ 0.007 & 17.866 $\pm$ 0.006 & 17.746 $\pm$ 0.008 & 17.723 $\pm$ 0.041 \\
217.931339 & 36.34208 & 19.812 $\pm$ 0.014 & 18.342 $\pm$ 0.008 & 16.818 $\pm$ 0.005 & 16.016 $\pm$ 0.007 \\
217.931216 & 36.27044 & 19.172 $\pm$ 0.010 & 18.382 $\pm$ 0.008 & 18.110 $\pm$ 0.009 & 17.988 $\pm$ 0.021 \\
217.918619 & 36.31995 & 20.742 $\pm$ 0.026 & 19.264 $\pm$ 0.013 & 18.483 $\pm$ 0.011 & 18.055 $\pm$ 0.024 \\
217.913905 & 36.28612 & 20.736 $\pm$ 0.027 & 19.266 $\pm$ 0.013 & 18.253 $\pm$ 0.010 & 17.687 $\pm$ 0.019 \\
217.928915 & 36.33948 & 20.850 $\pm$ 0.029 & 19.462 $\pm$ 0.017 & 18.214 $\pm$ 0.010 & 17.578 $\pm$ 0.018 \\
217.928801 & 36.30674 & 20.844 $\pm$ 0.028 & 19.471 $\pm$ 0.014 & 18.689 $\pm$ 0.012 & 18.315 $\pm$ 0.029 \\
217.955190 & 36.33084 & 19.708 $\pm$ 0.014 & 19.506 $\pm$ 0.015 & 19.505 $\pm$ 0.023 & 19.315 $\pm$ 0.065 \\
217.926000 & 36.33788 & 20.047 $\pm$ 0.016 & 19.640 $\pm$ 0.016 & 19.474 $\pm$ 0.022 & 19.437 $\pm$ 0.071 \\
217.932586 & 36.27256 & 21.248 $\pm$ 0.033 & 19.710 $\pm$ 0.016 & 18.342 $\pm$ 0.010 & 17.551 $\pm$ 0.016 \\
217.946853 & 36.30972 & 21.362 $\pm$ 0.040 & 19.909 $\pm$ 0.020 & 19.003 $\pm$ 0.016 & 18.439 $\pm$ 0.033 \\
217.971356 & 36.30059 & 21.318 $\pm$ 0.039 & 19.937 $\pm$ 0.020 & 19.043 $\pm$ 0.016 & 18.571 $\pm$ 0.035 \\
\enddata
\label{tab:sdssstars}
\end{deluxetable}
